A Unified View of Label Shift Estimation

Under label shift, the label distribution p(y) might change but the class-conditional distributions p(x|y) do not. There are two dominant approaches for estimating the label marginal. BBSE, a moment-matching approach based on confusion matrices, is provably consistent and provides interpretable error bounds. However, a maximum likelihood estimation approach, which we call MLLS, dominates empirically. In this paper, we present a unified view of the two methods and the first theoretical characterization of MLLS. Our contributions include (i) consistency conditions for MLLS, which include calibration of the classifier and a confusion matrix invertibility condition that BBSE also requires; (ii) a unified framework, casting BBSE as roughly equivalent to MLLS for a particular choice of calibration method; and (iii) a decomposition of MLLS's finite-sample error into terms reflecting miscalibration and estimation error. Our analysis attributes BBSE's statistical inefficiency to a loss of information due to coarse calibration. Experiments on synthetic data, MNIST, and CIFAR10 support our findings.

==> A Unified View of Label Shift Estimation (Neurips 2020)/sections/abstract.tex <==
% Faced with shifting label distributions but fixed class conditionals,
% we wish to estimate the target label distribution 
% given only unlabeled target samples.
% 
% 
    % Shall we define what label shift is?
    
    % Faced with shifting label distributions but fixed class conditionals,
    % two methods leverage black box classifiers to estimate 
    % the label marginal from labeled source and unlabeled target data. 
    % % The first, 
    % BBSE, a moment-matching approach based on confusion matrices, 
    % offers clean proofs of consistency and interpretable error bounds. 
    % % The second, 
    % However, MLLS, a maximum likelihood estimation approach 
    % that plugs in classifier outputs for the unknown $p(y|\mathbf{x})$, dominates empirically.
    % In this paper, we present a unified view of the two methods 
    % and the first theoretical characterization of the likelihood-based estimator.
    % Our contributions include (i) conditions for consistency of MLLS,
    % which include the calibration of the classifier and the very same 
    % confusion matrix invertibility condition required by BBSE;
    % (ii) a unified view of the methods casting the confusion matrix
    % as an instance of MLLS for a particular choice of calibration method;
    % and (iii) a decomposition of MLLS's error into terms reflecting 
    % the impacts of miscalibration and estimation error.
    % Our analysis attributes BBSE's inferior statistical efficiency
    % to a loss of information due to coarse calibration.
    % We support our findings with experiments on both synthetic data, 
    % MNIST, and the CIFAR10 image recognition datasets.
% image recognition dataset. 

 
% Label shift describes the setting where although the label distribution 
% might change between the source and target domains, 
% the class-conditional probabilities (of data given a label) do not. 
Under label shift, the label distribution $p(y)$ 
might change but the class-conditional distributions $p(x|y)$ do not.
There are two dominant approaches for estimating the label marginal. 
BBSE, a moment-matching approach based on confusion matrices, 
is provably consistent and provides interpretable error bounds. 
However, a maximum likelihood estimation approach, % (MLLS) 
which we call MLLS, dominates empirically.  
In this paper, we present a unified view of the two methods and 
the first theoretical characterization of MLLS.
% the likelihood-based estimator.  
Our contributions include 
(i) consistency conditions for MLLS, 
which include calibration of the classifier and a 
confusion matrix invertibility condition that BBSE also requires; 
(ii) a unified framework, casting 
% the confusion matrix approach
BBSE as roughly equivalent to MLLS 
for a particular choice of calibration method; 
and (iii) a decomposition of MLLS's finite-sample error into 
terms reflecting %the impacts of 
miscalibration and estimation error. 
Our analysis attributes BBSE's statistical inefficiency 
to a loss of information due to coarse calibration. 
% We support our findings with experiments on both synthetic data, 
% MNIST,and the CIFAR10 image recognition datasets.
% We support our findings with 
Experiments on synthetic data, MNIST, and CIFAR10 
% image recognition datasets.
support our findings.

% We support our findings experimentally, using both synthetic data and the CIFAR10 image recognition dataset


% (i) BBSE: a moment-matching approach
% based on confusion matrices; and 
% (ii) MLL: a maximum-likelihood estimator where the classifier's predictions are substituted for the (unknown) conditional probabilities $p(y|\x)$.
% % the likelihood of the data under the assumption that our classifier outputs true conditional probabilities.
% While BBSE boasts consistency and provable error bounds 
% % (assuming an invertibile confusion matrix),
% under mild assumptions,
% MLL's theoretical properties have not been characterized.
% % the coherence of LM method depends on the calibration of the classifier and
% % smooth it over
% % Moreover, to our knowledge, 
% % MLL's consistency conditions and error bounds
% % have not previously been established.
% % Despite lacking theoretical support, 
% % MLL outperforms BBSE empirically.
% However, empirical studies have suggested that when classifiers are per-class calibrated,
% MLL may outperform BBSE.
% % MLL in conjunction with per-label calibrated predictions appears to outperform BBSE empirically. 
% In this paper, we establish consistency conditions for MLL and establish error bounds, decoupling the contributions of miscalibration and estimation error. 
% Our work establishes a connection between the two approaches, clarifying how BBSE loses information due to its reliance on confusion matrix aggregates.
% We support our findings experimentally, using both synthetic data and the CIFAR10 image recognition dataset. 






% % Two popular methods address 
% Under label shift, we seek to estimate the label marginal $\pt(y)$ from unlabeled target data, assuming that the class-conditional $p(\x|y)$ remains fixed.
% Two popular methods exploit black box classifiers to address this problem:
% (i) BBSE: a moment-matching approach
% based on confusion matrices; and 
% (ii) MLL: a maximum-likelihood estimator where the classifier's predictions are substituted for the (unknown) conditional probabilities $p(y|\x)$.
% % the likelihood of the data under the assumption that our classifier outputs true conditional probabilities.
% While BBSE boasts consistency and provable error bounds 
% % (assuming an invertibile confusion matrix),
% under mild assumptions,
% MLL's theoretical properties have not been characterized.
% % the coherence of LM method depends on the calibration of the classifier and
% % smooth it over
% % Moreover, to our knowledge, 
% % MLL's consistency conditions and error bounds
% % have not previously been established.
% % Despite lacking theoretical support, 
% % MLL outperforms BBSE empirically.
% However, empirical studies have suggested that when classifiers are per-class calibrated,
% MLL may outperform BBSE.
% % MLL in conjunction with per-label calibrated predictions appears to outperform BBSE empirically. 
% In this paper, we establish consistency conditions for MLL and establish error bounds, decoupling the contributions of miscalibration and estimation error. 
% Our work establishes a connection between the two approaches, clarifying how BBSE loses information due to its reliance on confusion matrix aggregates.
% We support our findings experimentally, using both synthetic data and the CIFAR10 image recognition dataset. 
% % 

==> A Unified View of Label Shift Estimation (Neurips 2020)/sections/algorithm.tex <==

\begin{algorithm}
  \caption{Maximum Likelihood Label Shift estimation}
  \label{alg:MLLS}
%   \hspace*{\algorithmicindent} \textbf{Input}
\begin{algorithmic}[1]
  \INPUT: Labeled validation samples from source and unlabeled test samples from target. Trained blackbox model $\hat{\f}$, model class $\G$ and loss function $l$ for calibration (for instance, MSE or negative log-likelihood).
    \STATE On validation data minimize the loss $l$ over class $\G$ to obtain $\f = \g \circ \hat{\f}$. 
%   \STATE Initialize $noChange = true$.
%   \STATE Swap $x_i$ and $x_{i+1}$
  \STATE Solve the optimization problem \eqref{eq:mlls-sample} using $\f$ to get $\widehat \w$. 
  \OUTPUT: MLLS estimate $\widehat \w$ 
\end{algorithmic}
% \hspace*{\algorithmicindent} \textbf{Output}
\end{algorithm}


==> A Unified View of Label Shift Estimation (Neurips 2020)/sections/experiments.tex <==
	\label{sec:exp}

\begin{figure*}[t!] 
\centering
    % \setcounter{subfigure}{0}
    \subfigure[GMM]{ \includegraphics[width=0.3\linewidth]{sections/figures/gaussian_n_1000.png}}\hfil
    \subfigure[MNIST]{\includegraphics[width=0.3\linewidth]{sections/figures/MNIST_n_5000.png}}\hfil
    \subfigure[CIFAR-10]{\includegraphics[width=0.3\linewidth]{sections/figures/CIFAR_n_5000.png}}\par\medskip
    \vspace{-10pt}
    \subfigure[GMM]{\includegraphics[width=0.3\linewidth]{sections/figures/gaussian_alpha_0_99.png}}\hfil
    \subfigure[MNIST]{\includegraphics[width=0.3\linewidth]{sections/figures/MNIST_alpha_0_1.png}}\hfil
    \subfigure[CIFAR-10]{\includegraphics[width=0.3\linewidth]{sections/figures/CIFAR_alpha_0_1.png}}
    \vspace{-2pt}
\caption{ (\textbf{top}) MSE vs the degree of shift; For GMM, we control the shift in the label marginal for class 1 with a fixed target sample size of 1000. For multiclass problems----MNIST and CIFAR-10, we control the Dirichlet shift parameter with a fixed sample size of 5000. (\textbf{bottom}) MSE (in log scale) vs target sample size; For GMM, we fix the label marginal for class 1 at 0.01 whereas for multiclass problems, MNIST and CIFAR-10, we fix the Dirichlet parameter to 0.1. In all plots, MLLS dominates other methods. All confusion matrix approaches perform similarly, indicating that the advantage of MLLS  comes from the choice of calibration but not the way of performing distribution matching. 
%and the improvements are more pronounced for extreme shifts.   
% All plots and confidence intervals are obtained with 100 runs.
}\label{figure:MSE_err} 
\vspace{-13pt}
\end{figure*}

We experimentally illustrate the performance of MLLS on synthetic data, 
MNIST \citep{lecun1998mnist}, and CIFAR10 \citep{krizhevsky2009learning}. 
Following \citet{lipton2018detecting}, we experiment with \emph{Dirichlet shift} simulations.
On each run, we sample a target label distribution $\pt(y)$
from a Dirichlet with concentration parameter $\alpha$.
We then generate each target example by first sampling a label $y\sim \pt(y)$
and then sampling (with replacement) an example conditioned on that label .
% 
% 
% and the target data is sampled with replacement
% according to the 
% by first 
% data is sampled with replacement 
% with different tuning parameter $\alpha$ on the target label distribution.
Note that smaller values of alpha correspond to more severe shift.
In our experiments, the source label distribution is uniform.
% Unless specified otherwise, we assume the uniform source label distribution.    

First, we consider a mixture of two Gaussians (as in Example in Section~\ref{subsec:MLLS}) with $\mu=1$. 
With CIFAR10 and MNIST, we split the full training set into two subsets: 
train and valid, and use the provided test set as is.  
Then according to the label distribution,
we randomly sample with replacement train, valid, and test set 
from each of their respective pool to form the source and target set. 
To learn the black box predictor on real datasets, 
we use the same architecture as~\citet{lipton2018detecting} 
for MNIST, and for CIFAR10 we use ResNet-18~\citep{he2016deep} 
as in \citet{azizzadenesheli2019regularized}\footnote{We 
used open source implementation of ResNet-18 https://github.com/kuangliu/pytorch-cifar.}. 
For simulated data, we use the true $\ps(y|x)$ as our predictor function. 
For each experiment, we sample $100$ datasets 
for each shift parameter and evaluate the empirical MSE 
and variance of the estimated weights. 

We consider three sets of experiments: 
(1) MSE vs degree of target shift;
(2) MSE vs target sample sizes; 
and (3) MSE vs calibrated predictors on the source distribution. We refer to MLLS-CM as MLLS with hard confusion matrix calibration as in \eqref{eq:cm-log}. 
In our experiments, we compare MLLS estimator with BBSE, RLLS, and MLLS-CM. 
For RLLS and BBSE, we use the publicly available code \footnote{BBSE: https://github.com/zackchase/label\_shift, RLLS:  https://github.com/Angela0428/labelshift}. 
To post-hoc calibration, we use BCTS ~\citep{alexandari2019adapting} 
on the held-out validation set. 
Using the same validation set, we calculate 
the confusion matrix for BBSE, RLLS, and MLLS-CM. 

% \begin{figure}[bt!]

% \end{figure}

% We experimentally illustrate the performance of MLLS on synthetic data,
% MNIST \citep{lecun1998mnist}, and CIFAR10 \citep{krizhevsky2009learning}. 
% Following \citet{lipton2018detecting}, we experiment with \emph{Dirichlet shift} simulations for the target distribution keeping the source label distribution uniform. 
% First, we consider (synthetic data) a mixture of two Gaussians (as in Example in Section~\ref{subsec:MLLS} with $\mu=1$).  For simulated data, we use the true $\ps(y|x)$ as our predictor function. 
% To learn the black box predictor on real datasets, 
% we use the same architecture as~\citet{lipton2018detecting} 
% for MNIST, and for CIFAR10 we use ResNet-18~\citep{he2016deep} 
% as in \citet{azizzadenesheli2019regularized}.
% % \footnote{We used open source implementation of ResNet-18 https://github.com/kuangliu/pytorch-cifar.}
% More details about the experiments are included in Appendix~\ref{sec:exp_details}.
 
% We consider three sets of experiments: 
% (1) MSE vs degree of target shift;
% (2) MSE vs target sample sizes; 
% and (3) MSE vs calibrated predictors on the source distribution. Recall MLLS-CM is the MLLS analog with hard confusion matrix calibration as in \eqref{eq:cm-log}. 
% We compare MLLS estimator with BBSE, RLLS, and MLLS-CM. 
% For post-hoc calibration, we use BCTS ~\citep{alexandari2019adapting} 
% on the held-out validation set. 
% Using the same validation set, we calculate 
% the confusion matrix for BBSE, RLLS, and MLLS-CM. 




% Figure~\ref{figure:MSE} top row depicts the variation of MSE for different shifts in the target label distribution. 
We examine the performance of various estimators across all three datasets 
for various target dataset sizes and shift magnitudes (Figure~\ref{figure:MSE_err}).
Across all shifts, MLLS (with BCTS-calibrated classifiers)
\emph{uniformly dominates} BBSE, RLLS, and MLLS-CM 
in terms of MSE (Figure~\ref{figure:MSE_err}).
Observe for severe shifts, MLLS is comparatively dominant.
% Figure~\ref{figure:MSE} bottom row illustrates the variation of MSE with different sample sizes and fixed shift in the target distribution.
As the available target data increased, 
all methods improve rapidly,
with MLLS outperforming all other methods by a significant margin. 
% Confirming the findings of \citet{alexandari2019adapting}, 
Moreover, MLLS's advantages grow more pronounced under extreme shifts. 
Notice MLLS-CM is roughly equivalent to BBSE across all settings of dataset, target size, and shift magnitude. 
% Supporting our hypothesis that CM-log 
% (MLLS with CM calibration)
% is roughly equivalent to BBSE, the two methods
% perform similarly across all settings of dataset, target size, and shift magnitude.
This concludes MLLS's superior performance is not because of differences in loss function used for distribution matching but due to differences in the granularity of the predictions, caused by crude confusion matrix aggregation.  
% also demonstrate that the MSE of CM-Log is very close to that of BBSE and RLLS across different datasets, degree of shifts, and target sample sizes.  

\begin{wrapfigure}{r}{0.4\textwidth}
\vspace{-10pt}
  \centering 
%   \subfigure[]{\includegraphics[width=0.48\columnwidth]{sections/figures/Gaussian_bins-2.png}}
  \includegraphics[width=.33\columnwidth]{{sections/figures/gaussian_alpha_0_99_bins}.png} 
  \caption{ 
%   (a) Partition of $x$ and area for aggregation of predictor probabilities 
%   in the Gaussian mixture model with $2$ and $4$ equal sized bins,
%   Aggregation of prediction probabilities with the Gaussian mixture model with $2$ and $4$ bins,
MSE (left-axis) with variation of minimum eigenvalue of the Hessian (right-axis) vs number of bins used for aggregation.  With increase in number of bins, MSE decrease and the minimum eigenvalue increases.}\label{fig:Gbin}
\vspace{-10pt}
\end{wrapfigure}

% Note that predictors obtained by 
% using aggregation of any calibrated predictor 
Note that given a predictor $\f_1$,
we can partition our input space and produce another predictor $\f_2$ that, 
for any data-point gives the expected output of $\f_1$ 
on points belonging to that partition.
If $\f_1$ is calibrated, then $\f_2$ will also 
be calibrated \citep{vaicenavicius2019evaluating}.
% we obtain another calibrated predictor
% 
% over a partition of the input space gives another calibrated predictor \cite{vaicenavicius2019evaluating}.
% Note that predictors obtained using aggregation of any calibrated predictor 
% over a partition of the input space gives another calibrated predictor \cite{vaicenavicius2019evaluating}.
% 
On synthetic data, we vary the granularity of calibration (for MLLS)
% 
% \textcolor{red}{used for MLLS}
by aggregating $\ps(y|x)$ over a variable number of equal-sized bins. 
% Refer Figure \ref{fig:Gbin}(a) for visualization. 
% shows the variation of MSE and variation of the minimum eigenvalue of the empirical Hessian with an increasing number of bins which validates our theoretical results on the error bounds with a perfectly calibrated predictor.
% As the number of bins grows larger,
With more bins, less information is lost %by virtue of 
due to calibration.
Consequently, the minimum eigenvalue of the Hessian increases 
and the MSE decreases, supporting our theoretical bounds (Figure~\ref{fig:Gbin}).
% \textcolor{red}{
% Further,
% also verifies our claim of crude calibration with confusion matrix.
We also verify that the confusion matrix calibration
performs poorly (Figure~\ref{fig:Gbin}).
For MLLS-CM, the minimum eigenvalue of the Hessian is 0.195, 
% which is smaller than the minimum eigenvalue with 
significantly smaller than for the binned predictor for $\#$bin $\ge4$. 
Thus, the poor performance of MLLS-CM is predicted by
its looser upper bound per our analysis.
% This shows that the predictor obtained using confusion matrix calibration 
% has a loose upper bound, verifying the poor performance of confusion matrix approaches from our theoretical results.
% 
Note that these experiments presume access to the true predictor $\ps(y|x)$ and thus the MSE strictly improves with the number of bins. 
In practice, with a fixed source dataset size,
increasing the number of bins could lead to overfitting, worsening our calibration.

==> A Unified View of Label Shift Estimation (Neurips 2020)/sections/finite.tex <==
 \label{sec:finite}
 
We now analyze the MLLS estimators' convergence rates. For detailed proof from this section, we refer reader to Appendix \ref{sec:AppendixB}. 
Recall ${\widehat \w}$ denotes MLLS estimate~\eqref{eq:mlls-sample}. 
Let ${\w}^*$ denote the true shift. With consistency condition from section~\ref{subsec:MLLS}, we assume that $\w^*$ is the population minimizer with the calibrated predictor $\fc =  \ProbS({ y= . | \widehat \f(\x) })$ .i.e. 
\begin{align}
\w^* = &\argmax_{w \in \W} \E{\LL(\w; \fc )} \label{eq:MLLS_fc}
% &\quad \text{s.t.} \quad \sum_{y=1}^{k} w(y)\ps(y) = 1 \numberthis 
% &\quad \qquad \forall y \in \out \quad w(y) \ge 0 
\end{align}
 Our goal is to bound the finite sample error:  
\begin{equation}\label{eq:err}
    \Delta_n = ||\widehat \w - \w^*||_2 \le  \underbrace{||\widehat \w - \wc||_2}_{\RN{1}} +  \underbrace{||\wc - \w^*||_2}_{\RN{2}}  
\end{equation} 
where $ \wc$ is the finite sample estimation with the perfectly calibrated predictor $\fc$. We bound each error term on the RHS individually. Term-$\RN{1}$ denotes the estimation error due to finite sample re-calibration or inherent model misscalibration and term-$\RN{2}$ is the finite sample error with a perfectly calibrated model. 

% We use the following lemma
% % ~\ref{lemma:err_1} 
% to bound the error term-$\RN{2}$:  

\begin{lemma}[Error bound on term-$\RN{2}$]\label{lemma:err_1}
Assume the identifiability condition of lemma~\ref{lemma:identi-1} hold true and the predictor function  $\fc$ is bounded below at the non zero entries of $\w^*$ i.e. for all $\x$ such that $\pt(\x)>0$, we have $\sum_{y=1}^k \fc_y(\x) \w^*_y \ge \tau$ for some universal constant $\tau$. Let $\smin^{\fc}$ be the minimum eigenvalue of the Fisher information.  With probability at least $1-\delta$ we have,  
$$||\wc - \w^*||_2 \defeq \comp \left(\frac{1}{\smin^{\fc}}\sqrt{\frac{\log(\frac{4}{\delta})}{m}}\right)$$
\end{lemma}

\begin{proofsketch}

\end{proofsketch}


\begin{lemma}[Error bound on term-$\RN{1}$] \label{lemma:err_2}
Assume conditions from lemma \ref{lemma:err_1} hold true. Additionally assume the learnt predictor $\fh$ is also bounded below at the non zero entries of $\w^*$ i.e. for all $\x$ such that $\pt(\x)>0$, we have $\sum_{y=1}^k \fh_y(\x) \w^*_y \ge \tau$ for some universal constant $\tau$. Let $\smin^{\fh}$ be the minimum eigenvalue of the Fisher information with predictor $\fh$. With probability at least $1-\delta$ we have, 
\[
 || \wc - \widehat \w ||_2 \defeq \comp \left( \frac{1}{\sigma_{\min}^{\fh}}\Big(\sqrt{\frac{\log(\frac{4}{\delta})}{m}} +  \CE{\fh}||\w^*||_2 \Big) \right)
\]
\end{lemma}
\begin{proofsketch}

\end{proofsketch}

Depending on the degree of the miscalibration and method involved to calibrate $\fh$ we can bound the $\CE{\widehat \f}$. For example, if using vector scaling on a held out validation data from source for calibration, we can use lemma-\ref{lemma:platt} from Appendix \ref{sec:AppendixB} to bound the calibration error $\CE{\widehat \f}$ i.e. with standard regularity assumptions on model class $\G$ used for calibration we have with probability at least $1-\delta$,  
\begin{equation} \label{eq:platt}
  \CE{\fh} \le  \min_{\g \in \G} \CE{\g \circ \fh } + \sqrt{c\frac{\log(\frac{2}{\delta})}{n}}  
\end{equation}
  
\begin{theorem}[Error bounds] \label{thm:err}
Assume identifiability conditions of lemma \ref{lemma:identi-1} and assumption A.1 hold true. With probability at least $1-\delta$ we have, 
\begin{equation*}
\begin{split}
||\widehat \w - \w^*||_2  \defeq \comp \Bigg(\frac{1}{\smin^{\fc}}\sqrt{\frac{\log(\frac{4}{\delta})}{m}}  &+ \frac{1}{\sigma_{\min}^{\fh}}\Big(\sqrt{\frac{\log(\frac{4}{\delta})}{m}} \\ &+ \CE{\fh}||\w^*||_2 \Big) \Bigg)
\end{split}
\end{equation*}

\end{theorem}
The proof follows simply by combining above lemma's bounding the error terms $\RN{1}$ and $\RN{2}$ in \eqref{eq:err}. 

\todos[inline]{Remarks and takeaways from the above lemmas and theorem.}

\todos[inline]{Re-define the assumption from lemmas and justify that.}
To derive the finite sample bounds in lemma \ref{lemma:err_1} and \ref{lemma:err_2}, we make the following assumption: 

(A.1) \quad  


\textbf{Justification.} 
 
 
\todos[inline]{Explain what happens on the boundary} 

We begin this section by showing strong convexity of the log-likelihood. We need this condition for all our finite sample error analysis.

\begin{prop} \label{prop:strongconcave}
With the identifiability of the log-likelihood, the optimization problem~\eqref{eq:mlls-sample} is strongly convex.  
\end{prop}

The proof argument is detailed in Appendix-\ref{sec:AppendixB} the identifiability assumption. 


% \subsection{Generalization results} 
\todos{Majorly these will be from kamyar's paper which can be included for completeness.}


==> A Unified View of Label Shift Estimation (Neurips 2020)/sections/introduction.tex <==
% Despite their wide deployment, 
Supervised algorithms are typically developed and evaluated 
assuming independent and identically distributed (iid) data.  
However, the real world seldom abides,
presenting domain adaptation problems 
% characterized by mismatches between the 
in which the \textit{source distribution} $\ProbS$,
from which we sample labeled training examples, 
differs from the \textit{target distribution} $\ProbT$,
from which we only observe unlabeled data.
% 
Absent assumptions on the nature of shift, 
the problem is 
% Z: unnecessary
% fundamentally 
underspecified.
Multiple assumptions may be compatible 
with the same observations while implying
different courses of action.
% Fortunately, under invariances that naturally flow 
Fortunately, some assumptions can render 
shift detection, estimation, and on-the-fly updates 
to our classifiers possible.
% These assumptions often consist of invariances that
% Some such assumptions flow from causal structure \citep{scholkopf2012causal}.

% Formally, denoting our input features by $\x$ and labels by $y$, 
% two settings have been extensively studied.
This paper focuses on \emph{label shift}
\citep{storkey2009training, saerens2002adjusting, lipton2018detecting},
which aligns with 
% a hypothetical
the \emph{anticausal} setting 
in which the labels $y$ cause the features $\x$ \citep{scholkopf2012causal}.
% In the causal intepretation, an intervention 
Label shift arises in diagnostic problems
because diseases cause symptoms.
% In this interpretation, 
In this setting, an intervention on $p(y)$ induces the shift,
but the process generating $x$ given $y$ is fixed ($\ps(\x|y) = \pt(\x|y)$).
% Note that 
% in general, 
Under label shift, the optimal predictor 
% (based on $p(y|\x)$) 
may change,
% Given the same symptoms, 
e.g., the probability that a patient suffers from a disease
given their symptoms can increase under a pandemic.
% 
Contrast label shift with the better-known 
\emph{covariate shift} assumption, 
% which flows from the assumption that 
which aligns with the assumption that $\x$ causes $y$,
yielding the reverse implication that $\ps(y|\x) = \pt(y|\x)$.
% is invariant between the source and target distributions.
% In the causal interpretation, covariate shift 
% owes to selection bias on the covariates $\x$,
% but does not effect the ($x$-conditioned) process 
% by which labels are generated. 


Under label shift, our first task 
% is to
% relate the target and source distributions
% by estimating the likelihood ratios 
is to estimate the ratios
$w(y) = \pt(y)/\ps(y)$ for all labels $y$.
% for all labels $i$ with a predictive model $f$ trained on the source data.
% The problem may at first seem counter-intuitive, 
% because 
% Although we possess samples $y_i \sim \ps(y)$,
% we lack corresponding samples $y_j \sim \pt(y)$.
% 
% Z:  Add back next line only if we have space
% 
% Although we lack $y_j \sim \pt(y)$, the solution 
% may nevertheless be identifiable.
Two dominant approaches leverage off-the-shelf 
classifiers to estimate $\w$: (i) \emph{Black Box Shift Estimation} (BBSE) ~\citep{lipton2018detecting} and a variant called \emph{Regularized Learning under Label Shift} (RLLS)~\citep{azizzadenesheli2019regularized}: 
moment-matching based estimators that leverage 
(possibly biased, uncalibrated, or inaccurate) 
predictions to estimate the shift; 
% that that applies regularization when estimating the weights, giving small improvements;
and (ii) Maximum Likelihood Label Shift (MLLS) \citep{saerens2002adjusting}: 
an Expectation Maximization (EM) algorithm that 
% maximize the likelihood of observed unlabeled target data 
% estimates $\pt(y)$ but 
assumes access to a classifier that outputs
the true source distribution conditional probabilities~$\ps(y|\x)$.

%We also note that \citet{azizzadenesheli2019regularized} 
%propose a variant of BBSE called Regularised Learning under Label Shift (RLLS).
% under the source distribution. 
% 
%  Z: save our contributions for next paragraph
% 
% In this paper, we prove formally that this EM procedure 
% 
% 
% yields a maximum likelihood estimator.
% 
% yields a Maximum Likelihood Label Shift (MLLS) estimator.
% 
% 
% WHy we study MLLS? 
% 
% This line removed. 
% Maximum likelihood estimators have a rich history of asymptotic optimality as they achieve Cramer-Rao lower bound on the mean squared error~\cite{van2000asymptotic}. 
% 
% Assuming we possess 
Given a predictor $\smash{\widehat{\f}}$
with an invertible confusion matrix,
BBSE and RLLS have known consistency results
and finite-sample guarantees 
\citep{lipton2018detecting, azizzadenesheli2019regularized}.
However, 
% 
% absent rigorous theoretical guarantees,
% 
% lacking guarantees of consistency or convergence,
% despite lacking theoretical justification,
MLLS, in combination with
a calibration heuristic called Bias-Corrected Temperature Scaling (BCTS),
outperforms them empirically \citep{alexandari2019adapting}.

% applied to neural network predictors,
% MLLS outperforms RLLS and BBSE empirically. 

% statistical guarantees on consistency and rate of convergence are warranted on the moment matching approaches viz. BBSE and RLLS. 

In this paper, we theoretically characterize MLLS, 
establishing conditions for consistency 
and bounding its finite-sample error.
% However, until now, corresponding conditions 
% for consistency and finite-sample guarantees
% were unknown for the MLLS estimator.
% lacking for the likelihood-based approach questioning applicability of MLLS estimator. 
% Although, it is not hard to see that if we knew ground 
% While we can prove that if we could query 
To start, we observe that given the true label conditional $\ps(y|\x)$, 
MLLS is simply a concave Maximum Likelihood Estimation (MLE) problem 
% (not requiring EM) 
and standard results apply.
However, because we never know $\ps(y|\x)$ exactly, 
MLLS is always applied with an estimated model $\smash{\widehat{\f}}$ 
and thus the procedure consists of MLE under model misspecification.
% However, because we never know $\ps(y|\x)$ exactly, 
% MLLS is always applied with model misspecification.


% with poorly-characterized theoretical properties.
% ,
% relying on the predictor $f$ asa  $\ps(y|\x)$, 
% casting aspersions on its consistency. 


First, we prove that (i) \emph{\calib calibration} (Definition~\ref{def:calib}) 
and (ii) an invertible confusion matrix (as required by BBSE) 
% \todos{I think we need to re-write this based on lemma-1 and theorem-1. 
% Basically this depends on the chosen latent space. 
% Yifan please check this!!}
are \emph{sufficient conditions} to ensure MLLS's consistency (Proposition~\ref{prop:equiv-cond}, Theorems~\ref{theorem:mlls} and~\ref{theorem:convergence}).
% using binary classification as an example,
We also show that calibration can sometimes be \emph{necessary}
for consistency (Example~1 in Section~\ref{subsec:MLLS}). 
% 
% 
Recall that neural network classifiers tend to be uncalibrated 
absent post-hoc adjustments \cite{guo2017calibration}.
% To improve the MLLS estimate we need calibration 
% of the predictor $\smash{\widehat \f}$ 
% (discussed in Section~\ref{subsec:MLLS}). 
% 
Second, we observe that confusion matrices
can be instruments for calibrating a classifier. 
Applying MLLS with this technique,
BBSE and MLLS are distinguished only
by their objective functions. % that they optimize.
Through extensive experiments, 
we show that they
% that the two approaches
% show that the 
perform similarly, 
concluding that MLLS's superior performance
(when applied with more granular calibration techniques)
is not due to its objective but rather 
to the information lost by BBSE
via confusion matrix calibration. 
% 
Third, we analyze the finite-sample error 
of the MLLS estimator by decomposing its error into terms 
reflecting the miscalibration error and finite-sample error (Theorem~\ref{theorem:main-error-bound}). 
% Depending on the calibration technique involved, 
% we show how miscalibration error can be further divided 
% into the miscalibration error of the best model 
% and finite sample error to due incorporated method.
Depending on the calibration method, 
the miscalibration error can further be divided into two terms: 
finite sample error due to re-calibration on a validation set 
and the minimum achievable calibration error with that technique. 
% \todos{I have added pointers to specific theorems and definitions in the text for east reference. Is that fine? } 
% Should we include rates above in big O notation? 



We validate our results on synthetic data,
MNIST, and CIFAR-10.
% image recognition datasets. 
Empirical results show that MLLS can have
$2$--$10\times$ lower Mean Squared estimation Error (MSE)
% \todoy{I prefer to have some explicit measure, e.g. mse rather than "effective" when saying x-times more ...}
depending on the magnitude of the shift. 
% We experimentally characterize the variation of the
Our experiments relate MLLS's MSE 
% as a function of 
to the granularity of the calibration. 
% We show the variation of  MSE
% with varying ``sharpness'' viz. the refinement of the predictor
% as a function of the granularity of the calibration.  
% (here, the number of bins).
% \cite{kuleshov2015calibrated}.  
% How much extra experimentatl details should we add here? 
% I will add one more experiment that i am yet to run whcih shows the variation of MSE with miscalibration.  % Add a figure showing this. 

In summary, we contribute the following:
(i) Sufficient conditions for MLLS's consistency;
(ii) Unification of MLLS and BBSE methods under a common framework, 
with BBSE corresponding to a particular choice of calibration method;
    % and show how MLLS and BBSE are instantiated with this framework. Moreover we formulate confusion matrix as an instance of MLLS, which we refer to as CM-Log, for a particular choice of calibrated predictor, and loss function. 
(iii) Finite-sample error bounds for MLLS;  
    % \item We characterize and compare moment matching approaches with likelihood maximization in terms of the Fisher information matrix. % For example comparison of fisher information, aggregation is done in CM and how it affects the estimation error. 
(iv) Experiments on synthetic and image recognition datasets 
that support our theoretical arguments. 
    % Empirically, we contrast MLLS estimator with BBSL, RLLS, and CM-Log on synthetic and as well as on CIFAR-10 and MNIST datasets for various underlying target shifts, sample sizes, and calibrated predictors.  

% \raggedbottom
% \begin{enumerate}[itemsep=-.5ex,topsep=0pt]
%     % \item We show that \calib calibration of the predictor model on the source data along with the non-degeneracy of the confusion matrix are sufficient conditions for consistency of MLLS. 
%     \item Establishes sufficient conditions for MLLS' consistency.
%     % \item Unifies label shift estimation methods under a common framework, 
%     \item Unifies MLLS and BBSE methods under a common framework, 
%           with BBSE corresponding to a particular choice of calibration method.
%     % and show how MLLS and BBSE are instantiated with this framework. Moreover we formulate confusion matrix as an instance of MLLS, which we refer to as CM-Log, for a particular choice of calibrated predictor, and loss function. 
%     \item Derives finite-sample error bounds for MLLS.    
%     % \item We characterize and compare moment matching approaches with likelihood maximization in terms of the Fisher information matrix. % For example comparison of fisher information, aggregation is done in CM and how it affects the estimation error. 
%     \item Supports our theoretical arguments with extensive experiments
%     on synthetic and image recognition datasets. 
%     % Empirically, we contrast MLLS estimator with BBSL, RLLS, and CM-Log on synthetic and as well as on CIFAR-10 and MNIST datasets for various underlying target shifts, sample sizes, and calibrated predictors.  
% % \raggedbottom
% \end{enumerate}


% Despite their wide deployment, 
% supervised algorithms are typically developed and evaluated 
% assuming independent and identically distributed (iid) data.  
% However, the real world seldom abides,
% presenting domain adaptation problems 
% % characterized by mismatches between the 
% where the \textit{source distribution} $\ProbS$
% from which we sample labeled training examples 
% differs from the \textit{target distribution} $\ProbT$,
% from which we only observe unlabeled data.

% Absent assumptions on the nature of shift, 
% the problem is fundamentally under-specified.
% Multiple assumptions may be compatible 
% with the same observations while implying
% different courses of action.
% % Fortunately, under invariances that naturally flow 
% Fortunately, additional assumptions can render 
% shift detection, estimation, and on-the-fly updates 
% to our classifiers possible \citep{lipton2018detecting}.
% % These assumptions often consist of invariances that
% % Some such assumptions flow from causal structure \citep{scholkopf2012causal}.

% % Formally, denoting our input features by $\x$ and labels by $y$, 
% % two settings have been extensively studied.
% In this paper, we focus on \emph{label shift},
% which corresponds to the \emph{anticausal setting} \citep{scholkopf2012causal} 
% in which the labels $y$ causes the features $\x$ 
% \citep{storkey2009training, saerens2002adjusting, lipton2018detecting}.
% % In the causal intepretation, an intervention 
% Label shift arises in diagnostic problems,
% because diseases cause symptoms.
% In this interpretation, an intervention on $p(y)$ induces the shift,
% but the process generating $x$ given $y$ is fixed ($\ps(\x|y) = \pt(\x|y)$).
% Note that in general, under label shift, 
% the optimal predictor $p(y|\x)$ changes,
% % Given the same symptoms, 
% e.g., the probability that a patient suffers from a disease
% given their symptoms can increase under an epidemic.
% % 
% Contrast label shift with the better-known \emph{covariate shift} assumption, 
% % which flows from the assumption that 
% which flows from the $\x$ causes $y$ model,
% yielding the reverse implication that $\ps(y|\x) = \pt(y|\x)$.
% % is invariant between the source and target distributions.
% % In the causal interpretation, covariate shift 
% % owes to selection bias on the covariates $\x$,
% % but does not effect the ($x$-conditioned) process 
% % by which labels are generated. 


% Under label shift, our first task 
% % is to
% % relate the target and source distributions
% % by estimating the likelihood ratios 
% is to estimate the ratios
% $w(y) = \pt(y)/\ps(y)$ for all labels $y$.
% % for all labels $i$ with a predictive model $f$ trained on the source data.
% % The problem may at first seem counter-intuitive, 
% % because 
% % Although we possess samples $y_i \sim \ps(y)$,
% % we lack corresponding samples $y_j \sim \pt(y)$.
% % 
% % Z:  Add back next line only if we have space
% % 
% % Although we lack $y_j \sim \pt(y)$, the solution 
% % may nevertheless be identifiable.
% Two approaches leverage off-the-shelf 
% classifiers to estimate $\w$:
% (i) Black Box Shift Estimation (BBSE) ~\cite{lipton2018detecting}: 
% a moment-matching estimator that leverages 
% (possibly biased, uncalibrated, or inaccurate) 
% predictions to estimate the shift---\citet{azizzadenesheli2019regularized} 
% propose a variant called Regularised Learning under Label Shift (RLLS); 
% % that that applies regularization when estimating the weights, giving small improvements;
% and (ii) Maximum Likelihood Label Shift (MLLS): \citet{saerens2002adjusting} proposed an Expectation Maximization (EM) algorithm to 
% % maximize the likelihood of observed unlabeled target data 
% to estimate $\pt(y)$ under the assumption 
% that the classifier outputs true probabilities $\ps(y|\x)$.
% % under the source distribution. 
% % 
% %  Z: save our contributions for next paragraph
% % 
% % In this paper, we prove formally that this EM procedure 
% % 
% % 
% % yields a maximum likelihood estimator.
% % 
% % yields a Maximum Likelihood Label Shift (MLLS) estimator.
% % 
% % 
% % WHy we study MLLS? 
% % 
% % This line removed. 
% % Maximum likelihood estimators have a rich history of asymptotic optimality as they achieve Cramer-Rao lower bound on the mean squared error~\cite{van2000asymptotic}. 
% % 
% % Assuming we possess 
% Given a predictor $\widehat f$
% with an invertible confusion matrix,
% BBSE and RLLS are both provably consistent
% and offer finite-sample guarantees 
% \citep{lipton2018detecting, azizzadenesheli2019regularized}.
% However, absent known guarantees,
% % lacking guarantees of consistency or convergence,
% % despite lacking theoretical justification,
% MLLS was shown, in combination with Bias-Corrected Temperature Scaling (BCTS) to perform best empirically \citep{alexandari2019adapting}.

% % applied to neural network predictors,
% % MLLS outperforms RLLS and BBSE empirically. 

% % statistical guarantees on consistency and rate of convergence are warranted on the moment matching approaches viz. BBSE and RLLS. 

% This paper provides a theoretical analysis 
% of MLLS, establishing conditions for consistency 
% and bounding its finite-sample error.
% % However, until now, corresponding conditions 
% % for consistency and finite-sample guarantees
% % were unknown for the MLLS estimator.
% % lacking for the likelihood-based approach questioning applicability of MLLS estimator. 
% % Although, it is not hard to see that if we knew ground 
% % While we can prove that if we could query 
% To start, we observe that 
% % if we could access 
% given the true label conditional $\ps(y|\x)$, 
% % then the 
% MLLS is simply maximum likelihood estimation
% (not requiring EM)
% and standard theoretical results apply.
% However, because we never know $\ps(y|\x)$ exactly, MLLS is always applied with model misspecification.
% % with poorly-characterized theoretical properties.
% % ,
% % relying on the predictor $f$ asa  $\ps(y|\x)$, 
% % casting aspersions on its consistency. 

% First, we prove that (i) \emph{\calib calibration} 
% and (ii) invertible confusion matrix (as required by BBSE) 
% % \todos{I think we need to re-write this based on lemma-1 and theorem-1. 
% % Basically this depends on the chosen latent space. 
% % Yifan please check this!!}
% are \emph{sufficient conditions} to ensure MLLS' consistency.
% Moreover, using binary classification as an example,
% we prove that calibration can sometimes be  \emph{necessary}
% for consistency (see Example in Section~\ref{subsec:MLLS}). 
% % 
% Second, we make the observation that the confusion matrix 
% can be a (blunt) instrument for calibrating a classifier. 
% Given this calibration technique,
% the only difference between BBSE and MLLS is the objective function they optimize.
% Through extensive experiments, we show that the 
% two approaches perform similarly, concluding 
% that MLLS's superior performance
% (when applied with more granular calibration techniques)
% is not due to its objective but rather to the 
% information lost by the confusion matrix calibration. 
% % 
% Third, we theoretically analyze the finite-sample error 
% of the MLLS estimator by decomposing the error into terms 
% reflecting miscalibration error and finite sample error. 
% % Depending on the calibration technique involved, 
% % we show how miscalibration error can be further divided 
% % into the miscalibration error of the best model 
% % and finite sample error to due incorporated method.
% Depending on the calibration method, 
% miscalibration error can further be divided in to two terms: 
% finite sample error due to re-calibration on a validation set 
% and the minimum achievable calibration error with that technique.  
% % Should we include rates above in big O notation? 

% We validate our results on synthetic data
% and the MNIST and CIFAR-10 image recognition datasets. 
% Empirical results show that MLLS can have
% \textit{2-10x lower} Mean Squared estimation Error (MSE)
% % \todoy{I prefer to have some explicit measure, e.g. mse rather than "effective" when saying x-times more ...}
% depending on the magnitude of the shift. 
% We experimentally characterize the variation of 
% MSE with granularity of the calibration. 
% % We show the variation of  MSE
% % with varying ``sharpness'' viz. the refinement of the predictor
% % as a function of the granularity of the calibration.  
% % (here, the number of bins).
% % \cite{kuleshov2015calibrated}.  
% % How much extra experimentatl details should we add here? 
% % I will add one more experiment that i am yet to run whcih shows the variation of MSE with miscalibration.  % Add a figure showing this. 

% \textbf{Our key contributions are the following}:
% \begin{enumerate}[noitemsep,topsep=0pt]
%     % \item We show that \calib calibration of the predictor model on the source data along with the non-degeneracy of the confusion matrix are sufficient conditions for consistency of MLLS. 
%     \item Establish sufficient conditions for MLLS' consistency.
%     \item Unify label shift methods under a common framework, 
%             with BBSE corresponding to one calibration method.
%     % and show how MLLS and BBSE are instantiated with this framework. Moreover we formulate confusion matrix as an instance of MLLS, which we refer to as CM-Log, for a particular choice of calibrated predictor, and loss function. 
%     \item Derive finite-sample error bounds for MLLS.    
%     % \item We characterize and compare moment matching approaches with likelihood maximization in terms of the Fisher information matrix. % For example comparison of fisher information, aggregation is done in CM and how it affects the estimation error. 
%     \item Support our theoretical arguments with extensive experiments
%             on synthetic and image recognition datasets. 
%     % Empirically, we contrast MLLS estimator with BBSL, RLLS, and CM-Log on synthetic and as well as on CIFAR-10 and MNIST datasets for various underlying target shifts, sample sizes, and calibrated predictors.  
% % \raggedbottom
% \end{enumerate}


% % \textbf{Our key contributions are the following}:
% % \begin{enumerate}[noitemsep,topsep=0pt]
% %     % \item We show that \calib calibration of the predictor model on the source data along with the non-degeneracy of the confusion matrix are sufficient conditions for consistency of MLLS. 
% %     \item Establish sufficient conditions for MLLS' consistency.
% %     \item Unify framework for the label shift estimation methods and show how MLLS and BBSE are instantiated with this framework. Moreover we formulate confusion matrix as an instance of MLLS, which we refer to as CM-Log, for a particular choice of calibrated predictor, and loss function. 
% %     \item We provide theoretical analysis to derive finite-sample error bounds for the MLLS estimator.    
% %     % \item We characterize and compare moment matching approaches with likelihood maximization in terms of the Fisher information matrix. % For example comparison of fisher information, aggregation is done in CM and how it affects the estimation error. 
% %     \item Empirically, we contrast MLLS estimator with BBSL, RLLS, and CM-Log on synthetic and as well as on CIFAR-10 and MNIST datasets for various underlying target shifts, sample sizes, and calibrated predictors.  
% % % \raggedbottom
% % \end{enumerate}

% % \begin{figure}[t!]
% %   \centering
% %   \subfigure[MSE vs shift]{\includegraphics[width=0.48\columnwidth]{{sections/figures/gaussian_n_1000}.png}}
% %   \hfill
% %   \subfigure[$\log$(MSE) vs sample size]{\includegraphics[width=0.48\columnwidth]{{sections/figures/gaussian_alpha_0.99}.png}} 
  
% %   \subfigure[]{\includegraphics[width=\columnwidth]{{sections/figures/gaussian_alpha_0.99_bins}.png}
% %   } \label{fig:GMMbin}

% % %   \caption{\textbf{Validation on Simulated Data}: Mixture of Gaussian with 2 labels. Difference between MSE with different methods -- BBSE, RLLS, CM-log with the hard confusion matrix of the ground truth predictor, and MLLS with the truth predictions. 
% % %   (a) For a fixed sample size of 1000 variation of MSE with varying shift in target label distribution; (b) For a fix shift $[0.99, 0.01]$ in target distribution, variation of MSE with varying sample size used for estimation;
% % % (a) For a fixed sample size and shift, variation of MSE and minimum eigennvalue of the confusion matrix with varying number of bins used for agregation of true calibrated predictor.}
% % \end{figure}



% % approach to estimate label-shift with an appropriate bias-corrected calibration of the predictive model $f$. 
% % Even though calibration doesn't ensure recovery of true probability model, MLLS with calibrated predictor outperforms RLLS and BBSE. 
% % In this paper, we show that even if we can't recover the true probabilities $\ps(y|\x)$, \emph{per-label calibration} of the predictive model on the source is sufficient for the MLLS estimator to be consistent. 
% % For a simple binary classification task, we show that calibration is also necessary (Example~\ref{ex:necessary}). 



% % Next, we turn to analyse the discrepancy between the optimization objectives used by confusion matrix approaches in comparison to likelihood based method. 
% % In particular, we cast the confusion matrix as an instance of MLLS for a specific choice of crude calibration predictor generated by confusion matrix, which we refer to as CM-Log.
% % We show the superior performance of MLLS isn't due to the mismatch of objective functions but rather due to aggregation of predictor information in confusion matrix approaches. 
% % % How should we pitch the unified view above? 


% % Further, we theoretically analyze finite-sample error with the MLLS estimator by decomposing into error terms reflecting miscalibration error and estimation error with a perfectly calibrated predictor. Depending on the calibration technique involved, we show how miscalibration error can be futher divided into the miscalibration error of the best model and finite sample error to due incorporated method. 
% % % Should we include rates above in big O notation? 

% % We validate our results on synthetic data, and image recognition datasets -- MNIST and CIFAR-10. Empirical results show that the MLLS can be \textit{2-10x effective} in estimation depending on the degree of the shift in label distribution. 
% % We show the variation of Mean Squared estimation Error (MSE) with varying ``sharpness'' viz. the refinement of the predictor~\cite{kuleshov2015calibrated}.  
% % % How much extra experimentatl details should we add here? 
% % % I will add one more experiment that i am yet to run whcih shows the variation of MSE with miscalibration.  % Add a figure showing this. 
% % Our key contributions are summarized as following: 
% % \begin{itemize}[noitemsep,topsep=0pt]
% %     \item We show that per-label calibration of the predictor model on the source data is sufficient condition for consistency of MLLS. 
% %     \item We provide theoretical analysis to derive finite-sample error bounds for the MLLS estimator. 
% %     \item We give a unified view of the label shift estimation methods casting the confusion matrix as an instance of MLLS for a particular choice of calibrated predictor. 
% %     % \item We characterize and compare moment matching approaches with likelihood maximization in terms of the Fisher information matrix. % For example comparison of fisher information, aggregation is done in CM and how it affects the estimation error. 
% %     \item Empirically, we contrast MLLS estimator with BBSL, RLLS, and CM-Log on synthetic and as well as on CIFAR-10 and MNIST datasets for various underlying target shifts, sample sizes, and calibrated predictors.  
% % % \raggedbottom
% % \end{itemize}

% % \begin{figure}[t!]
% %   \centering
% % %   \subfigure[MSE vs shift]{\includegraphics[width=0.48\columnwidth]{{sections/figures/gaussian_n_1000}.png}\label{fig:Gn}}
% % %   \hfill
% % %   \subfigure[$\log$(MSE) vs sample size]{\includegraphics[width=0.48\columnwidth]{{sections/figures/gaussian_alpha_0.99}.png}
% % %   \label{fig:Galpha}} 
  
% %   \subfigure[]{\includegraphics[width=\columnwidth]{{sections/figures/gaussian_alpha_0.99_bins}.png}
% %   \label{fig:Gbin}}

% %   \caption{\textbf{Validation on Simulated Data}: Mixture of Gaussian with 2 labels. Difference between MSE with different methods -- BBSE, RLLS, CM-log with the hard confusion matrix of the ground truth predictor, and MLLS with the truth predictions. 
% % %   (a) For a fixed sample size of 1000 variation of MSE with varying shift in target label distribution; (b) For a fix shift $[0.99, 0.01]$ in target distribution, variation of MSE with varying sample size used for estimation;
% % (a) For a fixed sample size and shift, variation of MSE and minimum eigennvalue of the confusion matrix with varying number of bins used for agregation of true calibrated predictor.}
% % \end{figure}



% % % What is label shift
% % Most of the supervised machine learning today deals with independent and identically distributed (iid) data during training and testing. With this assumption supervised learning models have succeeded in achieving fairly decent accuracy on the unseen target data. But, what if there is a distribution shift among the test samples coming from a \textit{target distribution} $\T$, as compared to the training data coming from a fixed \textit{source distribution} $\Ss$. Can the models -- trained on data sampled from a specific source distribution -- still achieve high accuracy on a possibly unknown target data distribution? 
% % % Some motivation on why label shift? Left blank

% % Without any assumptions on the nature of shift, the problem is impossible to solve. However, under distribution shift assumptions some progress can be been made. Formally, if we denote $\x$ as the input features and $y$ as the output labels, there are two main settings; \textit{Covariate shift} where $p(y|\x)$ remains fixed among source and target but the prior distribution on features $\x$ changes. \textit{Label shift} where $p(\x|y)$ remains fixed but the prior distribution on labels $y$ changes among source and target. 

% % % Work on covariate shift vs label shift. 
% % Covariate shift has been explored a lot in the literature whilst the label shift has gained interest only recently and is sparsely studied area despite its wide applicability in the medical diagnosis of disease and recognition tasks. In this work, we primarily focus on the label-shift setting.  

% % % Work on label shift
% % The main task under label shift is to quantify prior probability shift ratios $w_i = \pt(y_i)/\ps(y_i)$ for all labels $i$ with a predictive model $f$ trained on the source data. There are two candidate approaches to tackle the problem: (i) Moment matching estimator, or Black Box Shift Learning (BBSL) ~\cite{lipton2018detecting} which uses the black box predictor which can be biased, uncalibrated, and possibly inaccurate to estimate the shift. ~\citet{azizzadenesheli2019regularized} proposed a variant Regularised Learning under Label Shift (RLLS) which uses regularization on the shift to improve over BBSL. (ii) Maximum Likelihood estimator (MLL),~\citet{saerens2002adjusting} proposed using Expectation maximization (EM) algorithm to maximize the likelihood of observed unlabeled target data to estimate the shift. 

% % % Edit this to show our contribution nicely maybe by adding a note at the end of the paragraph discerning our contribution with Bias corrected calibration work.   
% % % Can elaborate on asymptotics more. 
% % Maximum likelihood estimators have a rich history of asymptotic optimality as they achieve Cramer-Rao lower bound on the mean squared error~\cite{van2000asymptotic}. However for label-shift estimation, in practice, MLL is always dealing with model misspecification as it uses the predictor function $f$ instead of true distribution $\ps(y|\x)$. 
% % % With finite data, it is impossible to recover the true distribution $\ps(y|\x)$.
% % In this paper, we show that even if we can't recover the true probabilities $\ps(y|\x)$, \textit{per-label calibration} of the predictive model on the source is sufficient for the MLL estimator to be consistent. For a simple binary classification task, we show that calibration is also necessary (Example~\ref{ex:necessary}). 
% % Empirically, \citet{alexandari2019adapting} observed the effectiveness of the EM approach to estimate label-shift with an appropriate bias-corrected calibration of the predictive model $p(y|\x)$. 
  
% % Next, we turn to analyze finite-sample error with the MLL estimator. Strong statistical guarantees on consistency and rate of convergence are warranted on the moment matching approaches viz. BBSE and RLLS, but corresponding theoretical guarantees are lacking for the likelihood-based approach questioning applicability of MLL estimator. In this work, we analyze the properties of the likelihood optimization problem~\cite{saerens2002adjusting} and provide finite sample bounds on the rate of convergence of the error estimates. As a side, we also show that moment matching approaches, specifically the ones which use a hard thresholded predictor, in principle are constructing a calibrated classifier on the source data.

% % % Should we include characterization of the finite samples errors we have? 
% % % Should we include more on the problems with CM ie. it aggregates the information across samples and hence MLL can be a better choice in cases when we actually have sharp predictors. 


% % On synthetic data, we show that the likelihood approach can be \textit{10-30x effective in estimation} depending on the degree of the shift in label distribution. We run experiments on CIFAR-10 and MNIST with various calibrated predictors by varying the ``sharpness'' viz. the refinement of the predictor~\cite{kuleshov2015calibrated} and show how the estimation error varies with different choices of calibrated predictors. 
% % % Improve this
% % We conclude that confusion matrix approaches aggregate the predictor information across samples and hence MLL can be a better choice in cases when we actually have sharp predictors. 
% % % Add a figure showing this. 
% % % Add experiment details for real data and finalize the kinds of comparison we want. 
    

% % Our key contributions are following: 
% % \begin{itemize}[noitemsep,topsep=0pt]
% %     \item We show that per-label calibration of the predictor model on the source data is sufficient condition for consistency. 
% %     \item We provide theoretical analysis to derive finite-sample error bounds for the MLL estimator. 
% %     \item We characterize and compare moment matching approaches with likelihood maximization in terms of the Fisher information matrix. % For example comparison of fisher information, aggregation is done in CM and how it affects the estimation error. 
% %     \item Empirically, we show that the MLL estimator achieves much lower estimation error as compared to the moment matching approach on synthetic and as well as on CIFAR-10 and MNIST datasets.  
% % % \raggedbottom
% % \end{itemize}

% % I will fix sizes of the legend and axis. 




% % \begin{figure}[!tbp]
% %   \centering
% %   \subfigure[abc]{\includegraphics[width=0.48\columnwidth]{{sections/figures/squared_n_1000}.png}\label{fig:Sn}}
% %   \hfill
% %   \subfigure[xyz]{\includegraphics[width=0.48\columnwidth]{{sections/figures/squared_x_alpha_0.99}.png}
% %   \label{fig:Salpha}}
% %   \caption{Same figure as above but with $x^2$ as the data generating distribution. We can decide which to keep. I would suggest above because Gaussian example would be easily understandable and the performance difference is not too different. We can probability remove this or shift this to appendix}
% % \end{figure}




% \textbf{Our key contributions are the following}:
% \begin{enumerate}[noitemsep,topsep=0pt]
%     % \item We show that \calib calibration of the predictor model on the source data along with the non-degeneracy of the confusion matrix are sufficient conditions for consistency of MLLS. 
%     \item Establish sufficient conditions for MLLS' consistency.
%     \item Unify framework for the label shift estimation methods and show how MLLS and BBSE are instantiated with this framework. Moreover we formulate confusion matrix as an instance of MLLS, which we refer to as CM-Log, for a particular choice of calibrated predictor, and loss function. 
%     \item We provide theoretical analysis to derive finite-sample error bounds for the MLLS estimator.    
%     % \item We characterize and compare moment matching approaches with likelihood maximization in terms of the Fisher information matrix. % For example comparison of fisher information, aggregation is done in CM and how it affects the estimation error. 
%     \item Empirically, we contrast MLLS estimator with BBSL, RLLS, and CM-Log on synthetic and as well as on CIFAR-10 and MNIST datasets for various underlying target shifts, sample sizes, and calibrated predictors.  
% % \raggedbottom
% \end{enumerate}

% \begin{figure}[t!]
%   \centering
%   \subfigure[MSE vs shift]{\includegraphics[width=0.48\columnwidth]{{sections/figures/gaussian_n_1000}.png}}
%   \hfill
%   \subfigure[$\log$(MSE) vs sample size]{\includegraphics[width=0.48\columnwidth]{{sections/figures/gaussian_alpha_0.99}.png}} 
  
%   \subfigure[]{\includegraphics[width=\columnwidth]{{sections/figures/gaussian_alpha_0.99_bins}.png}
%   } \label{fig:GMMbin}

% %   \caption{\textbf{Validation on Simulated Data}: Mixture of Gaussian with 2 labels. Difference between MSE with different methods -- BBSE, RLLS, CM-log with the hard confusion matrix of the ground truth predictor, and MLLS with the truth predictions. 
% %   (a) For a fixed sample size of 1000 variation of MSE with varying shift in target label distribution; (b) For a fix shift $[0.99, 0.01]$ in target distribution, variation of MSE with varying sample size used for estimation;
% % (a) For a fixed sample size and shift, variation of MSE and minimum eigennvalue of the confusion matrix with varying number of bins used for agregation of true calibrated predictor.}
% \end{figure}



% approach to estimate label-shift with an appropriate bias-corrected calibration of the predictive model $f$. 
% Even though calibration doesn't ensure recovery of true probability model, MLLS with calibrated predictor outperforms RLLS and BBSE. 
% In this paper, we show that even if we can't recover the true probabilities $\ps(y|\x)$, \emph{per-label calibration} of the predictive model on the source is sufficient for the MLLS estimator to be consistent. 
% For a simple binary classification task, we show that calibration is also necessary (Example~\ref{ex:necessary}). 



% Next, we turn to analyse the discrepancy between the optimization objectives used by confusion matrix approaches in comparison to likelihood based method. 
% In particular, we cast the confusion matrix as an instance of MLLS for a specific choice of crude calibration predictor generated by confusion matrix, which we refer to as CM-Log.
% We show the superior performance of MLLS isn't due to the mismatch of objective functions but rather due to aggregation of predictor information in confusion matrix approaches. 
% % How should we pitch the unified view above? 


% Further, we theoretically analyze finite-sample error with the MLLS estimator by decomposing into error terms reflecting miscalibration error and estimation error with a perfectly calibrated predictor. Depending on the calibration technique involved, we show how miscalibration error can be futher divided into the miscalibration error of the best model and finite sample error to due incorporated method. 
% % Should we include rates above in big O notation? 

% We validate our results on synthetic data, and image recognition datasets -- MNIST and CIFAR-10. Empirical results show that the MLLS can be \textit{2-10x effective} in estimation depending on the degree of the shift in label distribution. 
% We show the variation of Mean Squared estimation Error (MSE) with varying ``sharpness'' viz. the refinement of the predictor~\cite{kuleshov2015calibrated}.  
% % How much extra experimentatl details should we add here? 
% % I will add one more experiment that i am yet to run whcih shows the variation of MSE with miscalibration.  % Add a figure showing this. 
% Our key contributions are summarized as following: 
% \begin{itemize}[noitemsep,topsep=0pt]
%     \item We show that per-label calibration of the predictor model on the source data is sufficient condition for consistency of MLLS. 
%     \item We provide theoretical analysis to derive finite-sample error bounds for the MLLS estimator. 
%     \item We give a unified view of the label shift estimation methods casting the confusion matrix as an instance of MLLS for a particular choice of calibrated predictor. 
%     % \item We characterize and compare moment matching approaches with likelihood maximization in terms of the Fisher information matrix. % For example comparison of fisher information, aggregation is done in CM and how it affects the estimation error. 
%     \item Empirically, we contrast MLLS estimator with BBSL, RLLS, and CM-Log on synthetic and as well as on CIFAR-10 and MNIST datasets for various underlying target shifts, sample sizes, and calibrated predictors.  
% % \raggedbottom
% \end{itemize}

% \begin{figure}[t!]
%   \centering
% %   \subfigure[MSE vs shift]{\includegraphics[width=0.48\columnwidth]{{sections/figures/gaussian_n_1000}.png}\label{fig:Gn}}
% %   \hfill
% %   \subfigure[$\log$(MSE) vs sample size]{\includegraphics[width=0.48\columnwidth]{{sections/figures/gaussian_alpha_0.99}.png}
% %   \label{fig:Galpha}} 
  
%   \subfigure[]{\includegraphics[width=\columnwidth]{{sections/figures/gaussian_alpha_0.99_bins}.png}
%   \label{fig:Gbin}}

%   \caption{\textbf{Validation on Simulated Data}: Mixture of Gaussian with 2 labels. Difference between MSE with different methods -- BBSE, RLLS, CM-log with the hard confusion matrix of the ground truth predictor, and MLLS with the truth predictions. 
% %   (a) For a fixed sample size of 1000 variation of MSE with varying shift in target label distribution; (b) For a fix shift $[0.99, 0.01]$ in target distribution, variation of MSE with varying sample size used for estimation;
% (a) For a fixed sample size and shift, variation of MSE and minimum eigennvalue of the confusion matrix with varying number of bins used for agregation of true calibrated predictor.}
% \end{figure}



% % What is label shift
% Most of the supervised machine learning today deals with independent and identically distributed (iid) data during training and testing. With this assumption supervised learning models have succeeded in achieving fairly decent accuracy on the unseen target data. But, what if there is a distribution shift among the test samples coming from a \textit{target distribution} $\T$, as compared to the training data coming from a fixed \textit{source distribution} $\Ss$. Can the models -- trained on data sampled from a specific source distribution -- still achieve high accuracy on a possibly unknown target data distribution? 
% % Some motivation on why label shift? Left blank

% Without any assumptions on the nature of shift, the problem is impossible to solve. However, under distribution shift assumptions some progress can be been made. Formally, if we denote $\x$ as the input features and $y$ as the output labels, there are two main settings; \textit{Covariate shift} where $p(y|\x)$ remains fixed among source and target but the prior distribution on features $\x$ changes. \textit{Label shift} where $p(\x|y)$ remains fixed but the prior distribution on labels $y$ changes among source and target. 

% % Work on covariate shift vs label shift. 
% Covariate shift has been explored a lot in the literature whilst the label shift has gained interest only recently and is sparsely studied area despite its wide applicability in the medical diagnosis of disease and recognition tasks. In this work, we primarily focus on the label-shift setting.  

% % Work on label shift
% The main task under label shift is to quantify prior probability shift ratios $w_i = \pt(y_i)/\ps(y_i)$ for all labels $i$ with a predictive model $f$ trained on the source data. There are two candidate approaches to tackle the problem: (i) Moment matching estimator, or Black Box Shift Learning (BBSL) ~\cite{lipton2018detecting} which uses the black box predictor which can be biased, uncalibrated, and possibly inaccurate to estimate the shift. ~\citet{azizzadenesheli2019regularized} proposed a variant Regularised Learning under Label Shift (RLLS) which uses regularization on the shift to improve over BBSL. (ii) Maximum Likelihood estimator (MLL),~\citet{saerens2002adjusting} proposed using Expectation maximization (EM) algorithm to maximize the likelihood of observed unlabeled target data to estimate the shift. 

% % Edit this to show our contribution nicely maybe by adding a note at the end of the paragraph discerning our contribution with Bias corrected calibration work.   
% % Can elaborate on asymptotics more. 
% Maximum likelihood estimators have a rich history of asymptotic optimality as they achieve Cramer-Rao lower bound on the mean squared error~\cite{van2000asymptotic}. However for label-shift estimation, in practice, MLL is always dealing with model misspecification as it uses the predictor function $f$ instead of true distribution $\ps(y|\x)$. 
% % With finite data, it is impossible to recover the true distribution $\ps(y|\x)$.
% In this paper, we show that even if we can't recover the true probabilities $\ps(y|\x)$, \textit{per-label calibration} of the predictive model on the source is sufficient for the MLL estimator to be consistent. For a simple binary classification task, we show that calibration is also necessary (Example~\ref{ex:necessary}). 
% Empirically, \citet{alexandari2019adapting} observed the effectiveness of the EM approach to estimate label-shift with an appropriate bias-corrected calibration of the predictive model $p(y|\x)$. 
  
% Next, we turn to analyze finite-sample error with the MLL estimator. Strong statistical guarantees on consistency and rate of convergence are warranted on the moment matching approaches viz. BBSE and RLLS, but corresponding theoretical guarantees are lacking for the likelihood-based approach questioning applicability of MLL estimator. In this work, we analyze the properties of the likelihood optimization problem~\cite{saerens2002adjusting} and provide finite sample bounds on the rate of convergence of the error estimates. As a side, we also show that moment matching approaches, specifically the ones which use a hard thresholded predictor, in principle are constructing a calibrated classifier on the source data.

% % Should we include characterization of the finite samples errors we have? 
% % Should we include more on the problems with CM ie. it aggregates the information across samples and hence MLL can be a better choice in cases when we actually have sharp predictors. 


% On synthetic data, we show that the likelihood approach can be \textit{10-30x effective in estimation} depending on the degree of the shift in label distribution. We run experiments on CIFAR-10 and MNIST with various calibrated predictors by varying the ``sharpness'' viz. the refinement of the predictor~\cite{kuleshov2015calibrated} and show how the estimation error varies with different choices of calibrated predictors. 
% % Improve this
% We conclude that confusion matrix approaches aggregate the predictor information across samples and hence MLL can be a better choice in cases when we actually have sharp predictors. 
% % Add a figure showing this. 
% % Add experiment details for real data and finalize the kinds of comparison we want. 
    

% Our key contributions are following: 
% \begin{itemize}[noitemsep,topsep=0pt]
%     \item We show that per-label calibration of the predictor model on the source data is sufficient condition for consistency. 
%     \item We provide theoretical analysis to derive finite-sample error bounds for the MLL estimator. 
%     \item We characterize and compare moment matching approaches with likelihood maximization in terms of the Fisher information matrix. % For example comparison of fisher information, aggregation is done in CM and how it affects the estimation error. 
%     \item Empirically, we show that the MLL estimator achieves much lower estimation error as compared to the moment matching approach on synthetic and as well as on CIFAR-10 and MNIST datasets.  
% % \raggedbottom
% \end{itemize}

% I will fix sizes of the legend and axis. 




% \begin{figure}[!tbp]
%   \centering
%   \subfigure[abc]{\includegraphics[width=0.48\columnwidth]{{sections/figures/squared_n_1000}.png}\label{fig:Sn}}
%   \hfill
%   \subfigure[xyz]{\includegraphics[width=0.48\columnwidth]{{sections/figures/squared_x_alpha_0.99}.png}
%   \label{fig:Salpha}}
%   \caption{Same figure as above but with $x^2$ as the data generating distribution. We can decide which to keep. I would suggest above because Gaussian example would be easily understandable and the performance difference is not too different. We can probability remove this or shift this to appendix}
% \end{figure}




==> A Unified View of Label Shift Estimation (Neurips 2020)/sections/prior.tex <==
\label{sec:prior} 
% \todos[inline]{The idea is to unify the IPMs basically squared error with MMD relating zhang et. al., lipton et. al. and kamyar et. al. We also not include this or shift to appendix in limit of pages? But the idea was also to have this paper as a unifying paper for these other papers. }
% Two broad approaches to this problem exist.
% have been explored to estimate the shift.
Two families of solutions have been explored that leverage a blackbox predictor:
BBSE \citep{lipton2018detecting}, 
a moment matching method,
% BBSE~\cite{lipton2018detecting}
uses the predictor $\smash{ \widehat \f}$ to compute a confusion matrix 
$\smash{ C_{\widehat{\f}} \defeq \ps(\widehat{y}, y) \in \Real^{k\times k}}$ on the source data. 
Depending on how $\smash{\widehat{y}}$ is defined, 
there are two types of confusion matrix for a predictor $\smash{\widehat{\f}}$: 
(i) the \emph{hard confusion matrix} $\smash{\widehat{y}=\argmax \widehat{\f}(\x)}$; and (ii) the \emph{soft confusion matrix}, where $\smash{\widehat{y}}$ is defined 
as a random prediction that follows 
the discrete distribution $\smash{\widehat{\f}(\x)}$ over $\smash{\out}$.
%The confusion matrix is estimated as 
%$[\widehat C_s]_{i,j} = \frac{1}{n} \sum_l \I{ \left({\argmax} \widehat \f(\x_l) = i\right) \land y_l = j}$. Correspondingly, we have soft confusion matrix where instead of argmax we aggregate the predictor vector itself. \todos{Yifan please have a look here for definition of soft confusion matrix}
Both soft and hard confusion matrix 
can be estimated from labeled source data samples.
The estimate $\smash{\widehat \w}$ is computed as 
$\smash{\widehat \w := \widehat C_{\widehat \f}^{-1} \widehat \mu}$, 
where $\smash{\widehat C_{\widehat{\f}}}$ is the estimate of confusion matrix and $\smash{\widehat\mu}$ is an 
estimate of $\smash{\pt(\widehat y)}$,
% 
% computed using the predictor $\widehat \f$ applied to the target data.
computed by applying the predictor $\smash{\widehat \f}$ to the target data.
% 
% $[\widehat \mu ]_j = \frac{1}{m} \sum_l \I{\argmax \widehat \f(\x_l) = j}$. 
In a related vein, RLLS~\citep{azizzadenesheli2019regularized} 
incorporates an additional regularization term of the form $\norm{\w - 1}$ 
and solves a constrained optimization problem 
%as in \citet{pires2012statistical} 
to estimate the shift ratios $\w$. 

% 
% They minimize MMD to match the kernel mean embeddings for the distributions
% $\pt(\x)$ and $\pt^\prime(\x) = \sum_{y \in \out} \pt(\x|y) \w(y) \ps(y) dy$.
% 
% Another way to estimates weights is to minimize
% the KL-divergence between the true data generating distribution
% and the assumed model class with the predictor function $\widehat \f(\x)$,
% KL-divergence seems a possible choice here because even without knowing the true data generating target distribution we can maximise a surrogate emp8irical loss\todos{Cite relevant work here}.
MLLS estimates $w$ as if performing maximum likelihood estimation,
but substitutes the predictor outputs for the true probabilities $\ps(y|\x)$.
% under the assumption that the predictor outputs true probabilities $p_S(y|\x)$
% yields the MLLS estimator.  
% Having no closed formed solution,
\citet{saerens2002adjusting}, who introduce this procedure,
describe it as an application of EM.
% Expected Maximization (EM) algorithm.   
% As we will show,
However, as observed in \citep{du2014semi, alexandari2019adapting}, 
% (see also Proposition~\ref{prop:convex}), 
the likelihood objective is concave, 
and thus a variety of %alternative iterative
optimization algorithms may be applied to recover the MLLS estimate.  
% 
\citet{alexandari2019adapting} also showed that MLLS underperforms BBSE when applied naively, a phenomenon that we shed 
more light on in this paper.
% Finally, we note the work of \citet{zhang2013domain} which proposed a 
% Maximum Mean Discrepancy (MMD) approach 
% to estimate $\w$. 
% \textbf{We present a more expansive review of related work in Appendix~\ref{sec:rel_work}}. 

% even when calibrating the classifier
% via temperature scaling~\cite{guo2017calibration},
% it dominates BBSE when the predictor is calibrated with BCTS.
% both MLLS, BBSE, and RLLS improve---with MLLS performing best.

% that temperature scaling~\cite{guo2017calibration} is insufficient to improve MLLS 
% whereas bias-corrected calibration of the classifier 
% improves both MLLS, BBSE, and RLLS---with MLLS performing best.

% Further, we characterize the per-label calibration as a sufficient condition for consistency.
% Add some statements strengthening our contributions by saying we provide more clarity on what's happening.  



==> A Unified View of Label Shift Estimation (Neurips 2020)/sections/setup.tex <==
\label{sec:pre}

Let $\inpt$ be the input space and 
$\out = \{1,2,\ldots, k\}$ the output space. 
Let $\ProbS, \ProbT : \inpt\times\out \to [0,1]$
be the source and target distributions
and let $\ps$ and $\pt$ denote the corresponding 
% probability density function or probability mass function. 
probability density (or mass) functions.
We use $\mathbb{E}_s$ and $\mathbb{E}_t$ to denote expectations 
over the source and target distributions. % respectively.  
% 
% Z: necessary? also seems to confuse RV with samples
% 
% By $\x \in \inpt$ and $y\in \out$, 
% we denote random variables sampled iid from the unknown source and target distribution. 
% Unlike standard supervised setting, 
In unsupervised domain adaptation, 
we possess labeled source data 
$\{(\x_1,y_1), (\x_2, y_2), \ldots , (\x_n, y_n)\}$ 
and unlabeled target data $\{\x_{n+1}, \x_{n+2}, \ldots, \x_{n+m}\}$. 
% \sbcomment{The old notation was bad so I changed it. Please see if anything else broke.}
% 
We also assume access to a black-box predictor %function 
$\smash{\widehat \f: \inpt \mapsto \Delta^{k-1}}$, e.g., 
a model trained to approximate 
the true probability function $f^*$, 
where $\smash{f^*(x) \defeq \ps(\cdot |\x)}$. 
% We also assume access to a black-box predictor function 
% $\widehat \f: \inpt \mapsto \Delta^{k-1}$, e.g., 
% a model trained to approximate the true probability function $\f^*: \inpt \mapsto \Delta^{k-1}$, 
% where $\f^*(\x) \defeq \ps(\cdot |\x)$. 
Here and in the rest of the paper, 
we use $\Delta^{k-1}$ to denote the standard $k$-dimensional probability simplex. 
For a vector $\vv$, we use $\vv_y$ 
to access the element at index $y$. 

% 
% Z: the lines below are a bit redundant (also already
    % mentioned in the introduction.
% 
% Practically, it is not possible 
% % Unfortunately, it is almost impossible \todoy{prefer not to say words like: unfortunately, almost impossible...} 
% to recover the true predictor function $\f^*(\x)$ with finite data and thus we assume $\widehat \f(\x)$ is some approximation $\widehat \ps(.|x)$. 

% Our objective is to learn a predictor 
% for the target distribution. 

Absent assumptions relating the source and target distributions,
domain adaptation is underspecified \citep{ben2010impossibility}.
% This paper works 
We work with the \emph{label shift} assumption, 
i.e., $\ps(\x|y) = \pt(\x|y)$,
focusing on multiclass classification.
Moreover, we assume non-zero support 
for all labels in the source distribution: 
for all $y \in \out$, $\ps(y) \ge c > 0$ \citep{lipton2018detecting,azizzadenesheli2019regularized}. 
Under label shift, three common goals are 
(i) detection---determining whether distribution shift has occurred;
(ii) quantification---estimating
the target label distribution; 
and (iii) correction---producing 
a predictor that minimizes error on the target distribution
\citep{lipton2018detecting}.
 
% as in ~\citet{lipton2018detecting}.
%
% ~\cite{lipton2018detecting} 
% 
% Z: commented out "discrete labels" because it's redundant with "multiclass classification"
% 
% with discrete labels.
% with known discrete label space.
% under the label shift assumption i.e. $\ps(\x|y) = \pt(\x|y)$.  
% With this assumption, 
% We wish to estimate the importance weights
This paper focuses on goal (ii),
estimating importance weights $w(y) = \pt(y)/\ps(y)$ 
for all $y \in \out$.
% using the predictor $\widehat \f(\x)$. 
% Quantification of shift enables
% Estimates of the target label distribution can be leveraged
% 
Given $\w$, we can update our classifiers on the fly,
either by retraining in an importance-weighted ERM framework \citep{shimodaira2000improving, gretton2009covariate, lipton2018detecting, azizzadenesheli2019regularized}---a practice 
that may be problematic for
overparameterized neural networks \citep{byrd2019effect},
% \sbcomment{include some more references here.}
or by applying an analytic correction
% using Bayes rule to predicted probabilities
% (this requires a calibrated classifier) 
\citep{alexandari2019adapting, saerens2002adjusting}.   
% \sbcomment{This last sentence is too terse and requires more explanation. What is the analytic correction? Why does it need calibration?}  
% \todos{Please check this.}
% 
% 
% We note that recent empirical results due to \citet{byrd2019effect} suggest 
% that retraining with importance weights 
% may not be an effective strategy for neural networks.
% \todos{Should we add something more here saying explicitly that we are not focusing on ERM or accuracy experiments and maybe add the Theorem 1 from the RLLS paper. }
% 
% 
% 
% \textcolor{red}{
% Moreover, with the ERM framework,
% Note with the ERM framework, 
Within the ERM framework, the generalization result from 
\citet{azizzadenesheli2019regularized} (Theorem 1)
depends only on the error of the estimated weights, 
and hence any method that improves weight estimates
tightens this bound. 
% is directly applicable to MLLS.
% They bound the generalization error by two terms: 
% one is bounded by a standard result on uniform laws
% % (doesn’t depend on the technique used to estimate shift);
% and the second is bounded by the estimation error on weights,
% where we can apply our Theorem \ref{theorem:main-error-bound} to get the rates. 
% Hence, improving weight estimates directly improves this bound.   

% \todos{Is putting calibration thing in the prior work fine, given we have some crucial definitions for the paper or should that go in problem setup? I have added here with 2 additional lines please check.}
% 
% 
% 
% 
% \textcolor{red}{Moreover, with the ERM framework, the generalization result from \citet{azizzadenesheli2019regularized} (Theorem 1) is directly applicable to MLLS.
% The generalization error in Theorem 1 \citep{azizzadenesheli2019regularized} is bounded by two terms: one is bounded by a standard result on uniform laws (doesn’t depend on the technique used to estimate shift); the second is bounded by the estimation error on weights, where we can apply our Theorem \ref{theorem:main-error-bound} to get the rates. Hence, improving weight estimates directly improves the generalization bound.  
% }
% 
% 
% 

% \textcolor{red}{
% 
%predictor $\smash{\widehat \f}$. Absent post-hoc adjustments, neural network predictions 
% which tend to
% 
% We introduce definitions and notation here.
% 

% In contrast to the setting of binary classification, 
There are multiple definitions of calibration in the multiclass setting.
%Calibration is clearly defined for binary classification % but 
% how best to unify the notion 
% how to define multiclass calibration
% for multiclass classification
% remains unclear 
% but there is no universal notion of 
%but multiple definitions of multiclass calibration exist
%\citep{vaicenavicius2019evaluating}.
\citet{guo2017calibration} study
%  the top-calibration error 
the calibration of the arg-max prediction,
while \citet{kumar2019verified} study a notion of 
per-label calibration.  
%which does not ensure \emph{reliability}~\citep{vaicenavicius2019evaluating}. 
% I can add details here, but should I?
%Instead, 
We use
%use the notion of 
\calib calibration~\citep{vaicenavicius2019evaluating}
and the expected \calib calibration error on the source data defined as follows:  
% \todos{I changed the definitions. Yifan could you please have a look.}
\begin{definition}[Canonical calibration]~\label{def:calib}
 A prediction model $\f: \mathcal{X} \mapsto \Delta^{k-1}$ is canonically calibrated  
 on the source domain 
 if for all $\x \in \inpt$ and $j \in \out$, 
%  \begin{align*}
 $\mathrm{P}_s ( y = j | \f(x) ) = \f_j(x) \,.$
%  \end{align*}
\end{definition}
% 
\begin{definition}[Expected \calib calibration error]~\label{def:caliberrr}
For a predictor $\f$, the expected squared \calib calibration error on the source domain is 
 $\smash{\mathcal{E}^2(f) =   \mathbb{E}_s \norm{\f - \fc}^2}$,
%  \CE{f} =  \left( \E{\sum_{j=1}^{k} \Big(f_j(\x) - P(y = j|f(\x))\Big)^2} \right)^{\frac{1}{2}}\,. \addeq\label{eq:caliberr}
 where $\smash{\fc = \mathrm{P}_s(y = \cdot |f(\x))}$.
%  \vspace{-5pt}
\end{definition}

Calibration methods typically work 
% One calibrates 
either by calibrating the model during training 
% while the
or by calibrating a trained classifier on held-out data, post-hoc.
We refer the interested reader to~\citet{kumar2019verified} and~\citet{guo2017calibration} for detailed studies on calibration. 
% for post-hoc calibration. 
We focus on the latter category of methods. Our experiments follow \citet{alexandari2019adapting},
who leverage BCTS \footnote{Motivated by the strong empirical results in \citet{alexandari2019adapting}, 
we use BCTS in our experiments as a surrogate to canonical calibration.}
% Bias-Corrected Temperature Scaling
to calibrate their models. BCTS extends temperature scaling~\citep{guo2017calibration} by incorporating 
per-class bias terms.
% \vspace{-8pt}

% Let the model class used for \emph{post-hoc calibration} be represented by $\G$. 
% Given a validation dataset $\{(x_{v1},y_{v1}),\ldots,(x_{vn},y_{vn})\}$ sampled from the 
% source distribution $P_s$ we compute,
% $\{(\widehat\f(\x_{v1}),y_{v1}), (\widehat\f(\x_{v2}), y_{v2}), \ldots , (\widehat\f(\x_{vn}), y_{vn})\}$, applying our
% classifier $\widehat{f}$ to the data.
% Using this we estimate
% %sampled iid from $\ProbS(\widehat\f(\x), y)$, 
% a function, 
% \begin{align}
% \widehat \g = \argmin_{\g \in \G} \sum_{i=1}^n \ell(\g \circ \widehat \f(\x_{vi}), y_{vi}) \,, \label{eq:posthoc}
% \end{align}
% where the loss function $\ell$ 
% can be the negative log-likelihood or squared error. 
% Subsequently, we can apply the calibrated predictor $\widehat{g} \circ \widehat{f}$. 
% In this paper, our focus is not on exploring calibration techniques. 

% We assume are given a black box predictor $f$, we incorporate calibration technique from the later class. 

% 
% Given a trained model $f$, 

 
% and a common scaling term across all classes. 
% Formally, a function $g:\Delta^{k-1} \mapsto \Delta^{k-1}$ in the BCTS class $\G$, is given by
% \begin{align*}
% g_j(x) = \frac{ \exp \left[ \log (x_j)/T + b_j\right] }{\sum_i \exp \left[ \log (x_i)/T + b_i \right ]} \quad \forall j \in \out \, 
% \end{align*}
% where $\{T, b_1,\ldots, b_{\abs{\out}}\}$
% are the $\abs{\out}+1$ parameters to be learned. 
% %

% Under the label shift setting, $w_{\x, y}$ are the importance weights $\w_y$. 
 
% 
% In the following, we briefly discuss the existing label shift estimation techniques and calibration techniques. 

% \subsection{} \label{subsec:bgd}
% {Prior Work on Label Shift Estimation}
% % \todos[inline]{The idea is to unify the IPMs basically squared error with MMD relating zhang et. al., lipton et. al. and kamyar et. al. We also not include this or shift to appendix in limit of pages? But the idea was also to have this paper as a unifying paper for these other papers. }
% % Two broad approaches to this problem exist.
% % have been explored to estimate the shift.
% Two families of solutions have been explored:
% BBSE \citep{lipton2018detecting}, 
% a moment matching method,
% % BBSE~\cite{lipton2018detecting}
% uses the predictor $\widehat \f$ to compute a confusion matrix 
% $C_{\widehat{\f}} \defeq \ps(\widehat{y}, y) \in \Real^{k\times k}$ on the source data. 
% Depending on how $\widehat{y}$ is defined, 
% there are two types of confusion matrix for a predictor $\widehat{\f}$: 
% (i) the \emph{hard confusion matrix} $\widehat{y}=\argmax \widehat{\f}(\x)$; and (ii) the \emph{soft confusion matrix}, where $\widehat{y}$ is defined 
% as a random prediction that follows 
% the discrete distribution $\widehat{\f}(\x)$ over $\out$.
% %The confusion matrix is estimated as 
% %$[\widehat C_s]_{i,j} = \frac{1}{n} \sum_l \I{ \left({\argmax} \widehat \f(\x_l) = i\right) \land y_l = j}$. Correspondingly, we have soft confusion matrix where instead of argmax we aggregate the predictor vector itself. \todos{Yifan please have a look here for definition of soft confusion matrix}
% Both soft and hard confusion matrix 
% can be estimated from labeled source data samples.
% The estimate $\widehat \w$ is computed as 
% $\widehat \w := \widehat C_{\widehat \f}^{-1} \widehat \mu$, 
% where $\widehat C_{\widehat{\f}}$ is the estimate of confusion matrix and $\widehat\mu$ is an 
% estimate of $\pt(\widehat y)$,
% % 
% % computed using the predictor $\widehat \f$ applied to the target data.
% computed by applying the predictor $\widehat \f$ to the target data.
% % 
% % $[\widehat \mu ]_j = \frac{1}{m} \sum_l \I{\argmax \widehat \f(\x_l) = j}$. 
% In a related vein, RLLS~\citep{azizzadenesheli2019regularized} 
% incorporates an additional regularization term of the form $\norm{\w - 1}$ 
% and solves a constrained optimization problem 
% %as in \citet{pires2012statistical} 
% to estimate the shift ratios $\w$.  

% % 
% % They minimize MMD to match the kernel mean embeddings for the distributions
% % $\pt(\x)$ and $\pt^\prime(\x) = \sum_{y \in \out} \pt(\x|y) \w(y) \ps(y) dy$.
% % 
% % Another way to estimates weights is to minimize
% % the KL-divergence between the true data generating distribution
% % and the assumed model class with the predictor function $\widehat \f(\x)$,
% % KL-divergence seems a possible choice here because even without knowing the true data generating target distribution we can maximise a surrogate emp8irical loss\todos{Cite relevant work here}.
% MLLS estimates weights as if performing maximum likelihood estimation,
% but substitutes the predictor outputs for the true probabilities $\ps(y|\x)$.
% % under the assumption that the predictor outputs true probabilities $p_S(y|\x)$
% % yields the MLLS estimator.  
% % Having no closed formed solution,
% \citet{saerens2002adjusting}, who introduce this procedure,
% describe it as an application of EM.
% % Expected Maximization (EM) algorithm.   
% % As we will show,
% However, as observed by \citet{alexandari2019adapting} (see also Proposition~\ref{prop:convex}), the likelihood objective is concave, 
% and thus a variety of alternative iterative optimization algorithms may be applied to recover the MLLS estimate.  
% % 
% \citet{alexandari2019adapting} also showed that MLLS underperforms BBSE when applied naively, a phenomenon that we shed 
% more light on in this paper.
% Finally, we note the work of \citet{zhang2013domain} which proposed a 
% Maximum Mean Discrepancy (MMD) approach 
% to estimate $\w$. 

% % even when calibrating the classifier
% % via temperature scaling~\cite{guo2017calibration},
% % it dominates BBSE when the predictor is calibrated with BCTS.
% % both MLLS, BBSE, and RLLS improve---with MLLS performing best.

% % that temperature scaling~\cite{guo2017calibration} is insufficient to improve MLLS 
% % whereas bias-corrected calibration of the classifier 
% % improves both MLLS, BBSE, and RLLS---with MLLS performing best.

% % Further, we characterize the per-label calibration as a sufficient condition for consistency.
% % Add some statements strengthening our contributions by saying we provide more clarity on what's happening.  

% \subsection{Calibration}
% % Recently, there have been growing interest in calibration methods  
% In contrast to the setting of binary classification, there are multiple 
% possible definitions of calibration in the multiclass setting.
% %Calibration is clearly defined for binary classification % but 
% % how best to unify the notion 
% % how to define multiclass calibration
% % for multiclass classification
% % remains unclear 
% % but there is no universal notion of 
% %but multiple definitions of multiclass calibration exist
% %\citep{vaicenavicius2019evaluating}.
% \citet{guo2017calibration} study
% %  the top-calibration error 
% the calibration of the arg-max prediction,
% while \citet{kumar2019verified} study a notion of 
% per-label calibration.  
% %which does not ensure \emph{reliability}~\citep{vaicenavicius2019evaluating}. 
% % I can add details here, but should I?
% %Instead, 
% We use
% %use the notion of 
% \calib calibration~\citep{vaicenavicius2019evaluating}
% and the expected \calib calibration error, which are 
% defined as follows:  
% % \todos{I changed the definitions. Yifan could you please have a look.}
% \begin{definition}[Canonical calibration]~\label{def:calib}
%  A prediction model $\f: \mathcal{X} \mapsto \Delta^{k-1}$ is canonically calibrated  
% %  in the source domain 
%  if for all $\x \in \inpt$ and $j \in \out$, 
%  \begin{align*}
%  \mathrm{P} ( y = j | \f(x) ) = \f_j(x) \,. \addeq\label{eq:calibdef}
%  \end{align*}
% \end{definition}
% % 
% \begin{definition}[Expected \calib calibration error]~\label{def:caliberrr}
% For a predictor $\f$, the expected \calib calibration error is  
%  \begin{align*}
%  \CE{f} =  \left( \mathbb{E} \norm{\f - \fc}^2 \right)^{\frac{1}{2}}\,, \addeq\label{eq:caliberr}
% %  \CE{f} =  \left( \E{\sum_{j=1}^{k} \Big(f_j(\x) - P(y = j|f(\x))\Big)^2} \right)^{\frac{1}{2}}\,. \addeq\label{eq:caliberr}
%  \end{align*}
%  where $\fc = \mathrm{P}(y = \cdot |f(\x))$.
% \end{definition}
% % 
% % Definition~\ref{def:calib} implies that %the distribution of the label 
% % the probability that the true label is $j$,
% % conditioned on the full vector of predicted probabilities $f$,
% % is equal to the predicted probability of the label $j$. 
% % This notion of calibration 
% % %is often referred to as
% % has been called
% % canonical calibration. 

% % We can elaborate on the motivation for Platt scaling
% Absent post-hoc adjustments, neural network predictions
% tend to be uncalibrated \cite{guo2017calibration}.
% % 
% % in general are uncalibrated. 
% % 
% % Broadly, there are two approaches to calibration.
% % obtain calibrated classifier.
% Calibration methods typically work 
% % One calibrates 
% either by calibrating the model during training 
% % while the
% or by calibrating a trained classifier on held-out data, post-hoc.
% % for post-hoc calibration. 
% We focus on the latter category of methods.
% Let the model class used for \emph{post-hoc calibration} be represented by $\G$. 
% Given a validation dataset $\{(x_{v1},y_{v1}),\ldots,(x_{vn},y_{vn})\}$ sampled from the 
% source distribution $P_s$ we compute,
% $\{(\widehat\f(\x_{v1}),y_{v1}), (\widehat\f(\x_{v2}), y_{v2}), \ldots , (\widehat\f(\x_{vn}), y_{vn})\}$, applying our
% classifier $\widehat{f}$ to the data.
% Using this we estimate
% %sampled iid from $\ProbS(\widehat\f(\x), y)$, 
% a function, 
% \begin{align}
% \widehat \g = \argmin_{\g \in \G} \sum_{i=1}^n \ell(\g \circ \widehat \f(\x_{vi}), y_{vi}) \,, \label{eq:posthoc}
% \end{align}
% where the loss function $\ell$ 
% can be the negative log-likelihood or squared error. 
% Subsequently, we can apply the calibrated predictor $\widehat{g} \circ \widehat{f}$. 
% % In this paper, our focus is not on exploring calibration techniques. 
% We refer the interested reader to~\citet{kumar2019verified} and~\citet{guo2017calibration} for detailed studies on calibration. 
% % We assume are given a black box predictor $f$, we incorporate calibration technique from the later class. 

% % 
% % Given a trained model $f$, 
% Our experiments follow \citet{alexandari2019adapting},
% who leverage BCTS \footnote{Motivated by the strong empirical results in \citet{alexandari2019adapting}, 
% we use BCTS in our experiments as a surrogate for canonical calibration.}
% % Bias-Corrected Temperature Scaling
% to calibrate their models. 
% BCTS extends temperature scaling~\citep{guo2017calibration} by incorporating 
% per-class bias terms. 
% % and a common scaling term across all classes. 
% Formally, a function $g:\Delta^{k-1} \mapsto \Delta^{k-1}$ in the BCTS class $\G$, is given by
% \begin{align*}
% g_j(x) = \frac{ \exp \left[ \log (x_j)/T + b_j\right] }{\sum_i \exp \left[ \log (x_i)/T + b_i \right ]} \quad \forall j \in \out \, 
% \end{align*}
% where $\{T, b_1,\ldots, b_{\abs{\out}}\}$
% are the $\abs{\out}+1$ parameters to be learned. 
% % \subsection{Notation and setup}
% Let $\inpt$ be the input space and 
% $\out = \{1,2,\ldots, k\}$ the output space. 
% Let $\ProbS, \ProbT : \inpt\times\out \to [0,1]$ 
% be the source and the target distributions. 
% By $\ps$ and $\pt$ we denote the corresponding 
% % probability density function or probability mass function. 
% probability density (or mass) functions. We use $\mathbb{E}_s$ and $\mathbb{E}_t$ to denote expectation over source and target marginals respectively.  
% % 
% % Z: necessary? also seems to confuse RV with samples
% % 
% % By $\x \in \inpt$ and $y\in \out$, 
% % we denote random variables sampled iid from the unknown source and target distribution. 
% % Unlike standard supervised setting, 
% In Domain Adaptation (DA), we possess labeled source data 
% $\{(\x_1,y_1), (\x_2, y_2), \ldots , (\x_n, y_n)\}$ 
% and unlabeled target data $\{\x_1, \x_2, \ldots, \x_m\}$. 
% % 
% We also assume access to a black-box predictor function 
% $\widehat \f(\x): \inpt \mapsto \Delta^{k-1}$, e.g. 
% % -- possibly uncalibrated, biased etc.\todoy{not sure what ``biased'' means here. also prob dont need to mention calibration here} -- 
% trained to approximate the true probability function 
% $\f^*(\x) \defeq \ps(y|\x)$. 

% % 
% % Z: the lines below are a bit redundant (also already
%     % mentioned in the introduction.
% % 
% % Practically, it is not possible 
% % % Unfortunately, it is almost impossible \todoy{prefer not to say words like: unfortunately, almost impossible...} 
% % to recover the true predictor function $\f^*(\x)$ with finite data and thus we assume $\widehat \f(\x)$ is some approximation $\widehat \ps(.|x)$. 

% % Our objective is to learn a predictor 
% % for the target distribution. 
% Two common objectives are (i) quantification---estimating
% the target label distribution, and (ii) correction---producing 
% a predictor that minimizes error on the target distribution.
% Absent assumptions relating the source and target distributions,
% % any problem of inference on the target distribution
% domain adaptation is underspecified \cite{ben2010impossibility}.
% % can be worst-case impossible as $\ProbS$ and $\ProbT$ might not share any support.  
% This paper addresses the \emph{label shift} assumption, 
% i.e., $\ps(\x|y) = \pt(\x|y)$,
% focusing on multiclass classification problems. Moreover, we assume non-zero support for all labels in the source distribution, i.e., for all $y \in \out$ $\ps(y) \ge c > 0$. 
% % as in ~\citet{lipton2018detecting}.
% %
% % ~\cite{lipton2018detecting} 
% % 
% % Z: commented out "discrete labels" because it's redundant with "multiclass classification"
% % 
% % with discrete labels.
% % with known discrete label space.
% % under the label shift assumption i.e. $\ps(\x|y) = \pt(\x|y)$.  
% % With this assumption, 
% % We wish to estimate the importance weights
% Our goal is to estimate important weights $w(y) = \pt(y)/\ps(y)$ 
% for all $y \in \out$.
% % using the predictor $\widehat \f(\x)$. 
% % Quantification of shift enables
% % Estimates of the target label distribution can be leveraged
% Given $\w$, we can update our classifiers on the fly,
% either by retraining with importance-weighted ERM framework---\citet{byrd2018effect}
% revealed that this may not be appropriate for deep networks---or 
% by applying an analytic correction to predicted probabilities
% (this requires a calibrated classifier). 

% % Under the label shift setting, $w_{\x, y}$ are the importance weights $\w_y$. 
 
% % 
% % In the following, we briefly discuss the existing label shift estimation techniques and calibration techniques. 

% % \subsection{} \label{subsec:bgd}

% \textbf{Label shift estimation  }
% % \todos[inline]{The idea is to unify the IPMs basically squared error with MMD relating zhang et. al., lipton et. al. and kamyar et. al. We also not include this or shift to appendix in limit of pages? But the idea was also to have this paper as a unifying paper for these other papers. }
% % Two broad approaches to this problem exist.
% % have been explored to estimate the shift.
% Two families of solutions have been explored:
% BBSE \citep{lipton2018detecting}, 
% a moment matching method,
% % BBSE~\cite{lipton2018detecting}
% uses the predictor $\widehat \f(\x)$ to compute a confusion matrix 
% $\mathbf{C}_{\hat{\f}} \defeq \ps(\hat{y}, y) \in \Real^{k\times k}$ on the source data. 
% Depending how $\hat{y}$ is defined, 
% there are two types of confusion matrix for a predictor $\widehat{\f}$: 
% (i) the \emph{hard confusion matrix} $\widehat{y}=\argmax \widehat{\f}(\x)$; and (ii) the \emph{soft confusion matrix}, where $\widehat{y}$ is defined 
% as a random prediction that follows 
% the discrete distribution $\widehat{\f}(\x)$ over $\out$.
% %The confusion matrix is estimated as 
% %$[\mathbf{\widehat C}_s]_{i,j} = \frac{1}{n} \sum_l \I{ \left({\argmax} \widehat \f(\x_l) = i\right) \land y_l = j}$. Correspondingly, we have soft confusion matrix where instead of argmax we aggregate the predictor vector itself. \todos{Yifan please have a look here for definition of soft confusion matrix}
% Both soft and hard confusion matrix 
% can be estimated from labeled source data samples.
% The estimate $\widehat \w$ is computed as 
% $\mathbf{\widehat C}_{\hat \f}^{-1} \widehat \mu$,
% where $\mathbf{\widehat C}_{\hat{\f}}$ is the estimate of confusion matrix and $\widehat\mu$ is the estimate of $\pt(\hat y)$. 
% % $[\widehat \mu ]_j = \frac{1}{m} \sum_l \I{\argmax \widehat \f(\x_l) = j}$. 


% RLLS~\citep{azizzadenesheli2019regularized} 
% incorporates the regularization term $\norm{\w - 1}_2$ 
% to solve a constrained optimization problem 
% as in \citet{pires2012statistical} 
% to estimate the shift ratios $\w$.  
% Previously, \citet{zhang2013domain} proposed a 
% Maximum Mean Discrepancy (MMD) approach 
% to estimate $\w$. 
% % 
% % They minimize MMD to match the kernel mean embeddings for the distributions
% % $\pt(\x)$ and $\pt^\prime(\x) = \sum_{y \in \out} \pt(\x|y) \w(y) \ps(y) dy$.
% % 
% % Another way to estimates weights is to minimize
% % the KL-divergence between the true data generating distribution
% % and the assumed model class with the predictor function $\widehat \f(\x)$,
% % KL-divergence seems a possible choice here because even without knowing the true data generating target distribution we can maximise a surrogate emp8irical loss\todos{Cite relevant work here}.
% MLLS estimates weights as if performing maximum likelihood estimation,
% but substitutes the predictor outputs for the true probabilities $\ps(y|\x)$.
% % under the assumption that the predictor outputs true probabilities $p_S(y|\x)$
% % yields the MLLS estimator.  
% % Having no closed formed solution,
% \citet{saerens2002adjusting}, who introduce this procedure,
% describe it as an application of EM.
% % Expected Maximization (EM) algorithm.   
% % As we will show,
% However, as we will show, the likelihood objective is convex, 
% and thus any iterative optimization algorithm % e.g., mirror descent, %or EM would 
% can recover the underlying MLLS estimate.  
% % 
% Recently, \citet{alexandari2019adapting} showed that 
% although MLLS underperforms BBSE when applied naively,
% % even when calibrating the classifier
% % via temperature scaling~\cite{guo2017calibration},
% % it dominates BBSE when the predictor is calibrated with BCTS.
% % both MLLS, BBSE, and RLLS improve---with MLLS performing best.

% % that temperature scaling~\cite{guo2017calibration} is insufficient to improve MLLS 
% % whereas bias-corrected calibration of the classifier 
% % improves both MLLS, BBSE, and RLLS---with MLLS performing best.

% % Further, we characterize the per-label calibration as a sufficient condition for consistency.
% % Add some statements strengthening our contributions by saying we provide more clarity on what's happening.  


% \textbf{Calibration  }
% % Recently, there have been growing interest in calibration methods  
% Calibration is clearly defined for binary classification % but 
% % how best to unify the notion 
% % how to define multiclass calibration
% % for multiclass classification
% % remains unclear 
% % but there is no universal notion of 
% but multiple definitions of multiclass calibration exist
% \citep{vaicenavicius2019evaluating}.
% \citet{guo2017calibration} study
% %  the top-calibration error 
% the calibration of the argmax prediction. 
% \citet{kumar2019verified} study per-label calibration.  
% %which does not ensure \emph{reliability}~\citep{vaicenavicius2019evaluating}. 
% % I can add details here, but should I?
% %Instead, 
% We use
% %use the notion of 
% \calib calibration~\citep{vaicenavicius2019evaluating}
% and the \calib expected calibration error defined as:  

% % \todos{I changed the definitions. Yifan could you please have a look.}
% \begin{definition}~\label{def:calib} (Canonical calibration)
%  A prediction model $\f$ is canonically calibrated  
% %  in the source domain 
%  if for all $\x \in \inpt$ and $j \in \out$, 
%  \begin{align*}
%  \mathrm{P} ( y = j | \f(x) ) = \f_j(x) \,. \addeq\label{eq:calibdef}
%  \end{align*}
% \end{definition}
% % 
% \begin{definition}~\label{def:caliberrr} (Expected \calib calibration error)
% For predictor $\f$, the expected \calib calibration error is  
%  \begin{align*}
%  \CE{f} =  \left( \E{\norm{\f - \fc}}^2 \right)^{\frac{1}{2}}\,, \addeq\label{eq:caliberr}
% %  \CE{f} =  \left( \E{\sum_{j=1}^{k} \Big(f_j(\x) - P(y = j|f(\x))\Big)^2} \right)^{\frac{1}{2}}\,. \addeq\label{eq:caliberr}
%  \end{align*}
%  where $\fc = \mathrm{P}(y = \cdot |f(\x))$
% \end{definition}
% % 
% % Definition~\ref{def:calib} implies that %the distribution of the label 
% % the probability that the true label is $j$,
% % conditioned on the full vector of predicted probabilities $f$,
% % is equal to the predicted probability of the label $j$. 
% % This notion of calibration 
% % %is often referred to as
% % has been called
% % canonical calibration. 

% % We can elaborate on the motivation for Platt scaling
% Absent post-hoc adjustments, neural network predictions
% tend to be uncalibrated \cite{guo2017calibration}.
% % 
% % in general are uncalibrated. 
% % 
% % Broadly, there are two approaches to calibration.
% % obtain calibrated classifier.
% Calibration methods typically work 
% % One calibrates 
% either by calibrating the model during training 
% % while the
% or post-hoc calibrating a trained classifier on held-out data.
% % for post-hoc calibration. 
% We focus on latter category of methods. 
% Let the model class used for \emph{post-hoc calibration} be represented by $\G$. 
% Given a validation dataset 
% $\{(\widehat\f(\x_1),y_1), (\widehat\f(\x_2), y_2), \ldots , (\widehat\f(\x_n), y_n)\}$ 
% sampled iid from $\ProbS(\widehat\f(\x), y)$,
% we output a function, 
% \begin{align}
% \widehat \g = \argmin_{\g \in \G} \sum_{i=1}^n l(\g \circ \widehat \f(\x_i), y_i) \,, \label{eq:posthoc}
% \end{align}
% where the loss function $l$ 
% can be negative log likelihood or squared error. 
% % In this paper, our focus is not on exploring calibration techniques. 
% We refer the interested reader to~\citet{kumar2019verified} and~\citet{guo2017calibration} for detailed studies on calibration. 
% % We assume are given a black box predictor $f$, we incorporate calibration technique from the later class. 
% % 
% % Given a trained model $f$, 
% Our experiments follow \citet{alexandari2019adapting},
% who leverage BCTS
% % Bias-Corrected Temperature Scaling
% to calibrate their models. 
% % \subsection{Other Related Work}
% % \input{sections/related.tex}

% % \begin{proof}

% % \end{proof}
% % This results is similar to Proposition-1 in recent work ~\cite{vaicenavicius2019evaluating}.


% \subsection{Other Related Work}
% \input{sections/related.tex}

% \begin{proof}

% \end{proof}
% This results is similar to Proposition-1 in recent work ~\cite{vaicenavicius2019evaluating}.


==> A Unified View of Label Shift Estimation (Neurips 2020)/sections/theory.tex <==
This section discusses our theoretical results -- 
% (i) we analyze the properties of the likelihood function, 
(i) necessary and sufficient conditions for consistency of MLLS, and (ii) finite sample error bounds for MLLS.  


The log-likelihood of observing \allowdisplaybreaks{$ \x_1, \x_2, \ldots, \x_m \stackrel{iid}{\sim} \pt(x)$} under the true model is given by 
%\todos[inline]{We can possibly shift this to appendix.}
\begin{align*}
\LL_m(\w, \f^*) &= \sum_{i=1}^m \log \pt(\x_i)\\
&\stackrel{i}{=} \sum_{i=1}^m \log \sum_{y\in\out} \pt(\x_i|y)\pt(y)   \\
&\stackrel{ii}{=} \sum_{i=1}^m \log \sum_{y\in\out} \ps(\x_i|y)\pt(y) \\
&= \sum_{i=1}^m \log \sum_{y\in\out} \ps(y|\x_i)\frac{\pt(y)}{\ps(y)} + \sum_{i=1}^m \log p_s(\x_i)
\end{align*}

where $(i)$ follows with Bayes theorem and $(ii)$ follows due to the label shift assumption. From now on, we ignore the term $\sum_{i=1}^m \log p_s(\x_i)$ as it is independent of the underlying parameters. 
We refer population log-likelihood as $\LL(\w, \f) = \E{\log\inner{\f(\x)}{\w} }$ and define the empirical log-likelihood as \allowdisplaybreaks{$\LL_m(\w; \widehat \f) =  \sum_{i=1}^m \log \sum_{y\in\out} \widehat \ps(y|\x_i)w(y) = \sum_{i=1}^m \log \inner{\widehat \f(\x_i)}{\w} $} which uses the predictor function $\widehat \f$ instead of the true marginal distribution.

We estimate the weights $\w$  i.e. the shift in the label distribution by maximizing the empirical log-likelihood (or minimizing the negative log-likelihood) 
\begin{align*}
\widehat \w = &\argmin_w - \LL_m(\w; \widehat \f ) \\ 
&\quad \text{s.t.} \quad ~\sum_{y=1}^{k} w(y)\ps(y) = 1 \numberthis \label{optprob}\\ 
&\quad \qquad \forall y \in \out \quad w(y) \ge 0 
\end{align*}

The above optimization problem is convex in nature as shown below. 
Under the assumption of non-zero support of source labels i.e. for all $y \in \out$ $\ps(y) = c > 0$ , the likelihood objective is also bounded above by $-\log(c)$. 
% In Appendix~\ref{sec:AppendixB}, we also show that the optimization problem is also self concordant (Proposition~\ref{prop:sc}). 
\begin{prop} The optimization problem defined in \eqref{optprob} is convex in nature.
\end{prop}
The proof argument follows simply. The objective function is negative log, a convex combination of a linear function in parameters. The minimization is over a convex region i.e. a simplex of dimensions $k-1$, and hence the overall optimization problem is convex.   

\textbf{Methods to maximise the likelihood.}
The optimization problem defined in \eqref{optprob} doesn't  
% Want to connvey unsurety 
seem to have a closed form solution but due to convexity and upper boundedness, we can use iterative procedures to find the MLLS estimate. In particular, we employ Expectation Maximisation (EM)~\cite{saerens2002adjusting} and mirror descent~\cite{beck2003mirror} on the likelihood function and observe same estimates empirically at the convergence of the iterates.    


% \todos{Ask if we should include formulation of EM and mirror descent. If needed I can add those.}

\subsection{Consistency of the estimate}\label{subsec:consistency}
In this subsection we formalize conditions on the predictor function $\widehat \f$ under which the optimization objective~\eqref{optprob} is identifiable, and the corresponding MLLS estimate is consistent.  

% \textbf{Motivating Scenario.}
% We begin with an example of binary classification problem on a mixture of two Gaussians where we show that calibration is necessary to achieve zero estimation error. To motivate the need for calibration we relate estimation error with the miscalibration error.  
% % with a simple Gaussian mixture model. 


% \begin{example} \label{ex:necessary}
% Consider a mixture of two Gaussians with \allowdisplaybreaks{$\ps(x|y=0) \defeq \N(\mu, 1)$ and $\ps(x|y=1) \defeq \N(-\mu, 1)$}. Assume source mixing coefficients be $\frac{1}{2}$ each and target mixing coefficients be $\alpha (\ne \frac{1}{2}), 1-\alpha $. Assume a class of probabilistic classifiers with threshold at $x=0$ that can be represented as $f(x) = [ \frac{1+(2c-1)\sign(x)}{2}, \frac{1-(2c-1)\sign(x)}{2}]$ with $c \in [0,1]$.  For such classifiers, the estimation error of population MLLS is given by $4\abs{\frac{\pt(x\le0) - c}{1-2c} - \alpha} = 4\abs{\frac{(1-2\alpha)(\ps(x\ge0|y=0) - c)}{1-2c}}$ which is zero for only if $c = \ps(x\ge0|y=0)$ for a non-degenerate classifier. 
% \end{example}

% % We extend the construction to probabilistic thresholded classifier in Appendix-\ref{sec:AppendixA}.   

% % Why such construction: 
% The intuition behind the construction is, for such problems, we can get a closed form expression for the population MLLS estimator and hence analyse the error theoretically. The expression for estimation error in the example gives two key insights; 
% % The main take away from this example is 
% One, uncalibrated thresholded classifier has an estimation error proportional to the true shift in label distribution  i.e. $1-2\alpha$.
% and two, the error is also proportional to degree of miscalibration which is $\ps(x\ge0|y=0) - c$. We formally derive the expression for estimation error in Appendix-\ref{sec:AppendixA}. 

% In the example below, we show that for any shift in the label distribution estimation error of the population MLLS estimator is directly propotional to the miscalibration error of the predictor function. 
% This gives some intuition on why calibration might be necessary but we leave a formal proof for this argument as future work.  

We now turn our discussion to
sufficient 
conditions for consistency.
\todos[inline]{I am not editing remaining of the subsection right now. We can discuss and decide what I should edit in this subsection.}

% \begin{prop}\label{prop:ident}
% (Identifiability condition.) Log-likelihood \allowdisplaybreaks{$\LL_m(\w; \widehat \f )$} is identifiable iff the matrix \allowdisplaybreaks{$\mathrm{\widehat P} = [\widehat \f(\x_1) \ldots \widehat \f(\x_n)]_{(k\times n)}$} formed by considering $\widehat \f(\x_i|y)$ for all $i\in \{1,\ldots,n\}$ and $y \in \out$ in the training data is full row-rank\footnote{Be default we assume we observe samples n greater than number of classes $\abs{\out}$}.
% \end{prop}
% % \todos[inline]{Ask how to handle continuos cases. }
% \begin{proof}
% Let's assume $\bm{q_1}, \bm{q_2}$ be vectors lying in $k-1$ dimentional simplex. With identifiability condition, if \allowdisplaybreaks{$ \bm{q_1} \ne \bm{q_2}$} then it must be the case that $\widehat \LL (\w_1; \x) \ne \widehat \LL_m(\w_2; \x)$. 

% Consider any arbitrary set $\x_1, \ldots, \x_n$ in the training data, log-likelihoods can only match when \allowdisplaybreaks{$[\widehat \f(\x_1) \ldots \widehat \f(\x_n)]^T \bm{q_1} = [\widehat \f(\x_1) \ldots \widehat \f(\x_n)]^T  \bm{q_2}$}. 
% Hence by rank-nullity theorem, full row-rank $\mathrm{\widehat P}$ implies identifiability.  
% \end{proof}
% \todos[inline]{I can add a detailed proof if it is required. We just need to add justification for what will happen if $\pt(x)$ is zero for some x. }

As the parameter $\w$ is restricted to a compact set, proposition
% -\ref{prop:ident} 
also implies strong identifiability.
% ~\cite{lecturenotes}. 
Full rank of $\mathrm{\widehat P}$ is also implied by full rank of the confusion matrix considered in \cite{lipton2018detecting}, but identifiability requires a weaker condition. 
Similar to proposition
% -\ref{prop:ident}
, we also need identifiability on the true log-likelihood which requires the true predictor function $\ps(y|\x)$ to be full rank on the source data. 


For consistency, we also need uniform law of large numbers condition on the log-likelihood which boils down to showing decaying Rademacher complexity on the approximate log-likelihood function class
% ~\cite{lecturenotes}
. We detail this argument in the appendix \ref{sec:AppendixA}.  

% \begin{lemma}\label{lemma:RC} (Rademacher complexity) Under certain assumptions viz.  boundedness etc. on the predictor function $\widehat \f$, the Rademacher complexity is 
% \begin{align*}
%  \R(\LL_m(\widehat \f )) = \mathbb{E}_{\x,\epsilon} &\Big[ \sup_{\w} \frac{1}{n} \sum_{i=1}^n \epsilon_i \log \inner{\widehat \f(\x_i)}{\w}  \Big] \\
%  &\defeq \comp(\frac{1}{\sqrt{m}})
% \end{align*}
% \end{lemma}

% \begin{lemma} [\cite{lecturenotes} Uniform LLN] As the log-likelihood function is continuous over the closed and bounded space of weight parameters and $\E{\sup_{\w} |\L_1(\x, \w ,\f)|}$ exists\footnote{This is finite for all $\w$'s that have a support for all non-zero $\w^*$'s}, we have uniform convergence on the empirical log-likelihood. 

% \end{lemma}



\begin{lemma}[Uniform Convergence~\cite{andersen1982cox}] \label{lemma:uc}
Suppose a sequence of convex function $\LL_m(\w, \f)$ converges in probability to $\LL(\w, \f)$ for $w$ in an open set $\mathcal{W}$, then $\sup_{\mathcal{W}^\prime} \abs{\LL_m(\w, \f) - \LL(\w, \f)}$ goes to zero in probability on every compact subset $\mathcal{W}^\prime$ of $\mathcal{W}$.     
\end{lemma}


\begin{lemma} [Consistency] With compact parameter space, continuity of the objective function, uniform convergence, and unique maxima, the MLL estimator is consistent.
\end{lemma}
\todos{For unique maxima we need identiability on the source data i.e. the predictor matrix being invertible. }


% Refer to Appendix~\ref{sec:AppendixA} for proof details. The argument uses Lipschitzness property and composition of Rademacher complexity. 

In any practical setting, with finite amount of data we can never estimate the true predictor $\ps(y|x)$ which leads to misspecified likelihood model. Thus, at the population level the MLE estimate would be the KL projection of true data generating distribution on our model.
% ~\cite{lecturenotes}. 
With per label calibration of the predictor function on the source data, we show that such model mis-specification is harmless. 
% First we give the definition of the \textit{per-label calibration} and then show the consistency of the MLE estimate.  


\begin{lemma} \label{lemma:consistency}
Suppose a predictor $\f$ is per-label calibrated and some identifiability condition, then true model $\LL (\w^*, \f^*)$ lies in the model class $\LL (\w, \f) $.
\end{lemma}
\begin{proof}
\todos[inline]{Add proof for the binary case}

\todos[inline]{Add the full-rank assumption of $\ps(\f(\x)|y)$ for identifiability.}
\end{proof}

In  Appendix \ref{sec:AppendixA}, we extend the proof to multiclass classification with continuos probabilities. \todos{Discuss with Yifan and add. }  

\begin{theorem}\label{theorem:con}
Assume per-label calibration and likelihood identifiability conditions hold, then the MLE is consistent. 
\end{theorem}  

% The proof follows by combining proposition~\ref{prop:ident}, lemma~\ref{lemma:RC}, and lemma~\ref{lemma:consistency}. The proof is formally compiled in Appendix \ref{sec:AppendixA}. 

We conclude that calibration is sufficient for consistency. Example-\ref{ex:necessary} gives intuition on why calibration might also be necessary but we leave a formal proof for this argument as future work.  
% \begin{example}\la
% Consider a mixture of Gaussian with \allowdisplaybreaks{$\ps(x|y=1) \defeq \N(1, 1)$ and $\ps(x|y=-1) \defeq \N(-1, 1)$}. Let source mixing coefficients be $\frac{1}{2}$ each and $\alpha, 1-\alpha$ be the target mixing coefficients. With any thresholded classifier of the form $f(x) = [ \frac{1+\sign(x)}{2}, \frac{1-\sign(x)}{2}]$, the estimation error is $4\abs{\pt(x\ge0) - \alpha} = 4\times 0.1587\abs{1 - 2\alpha}$ which is non-zero for all $\alpha \ne \frac{1}{2}$
% \end{example}


\subsection{Unified View}\label{subsec:unified}

Rather, one could also incorporate the predictor generated using the confusion matrix which in principle is calibrated (Proposition~\ref{prop:calib}). In section ~\ref{sec:exp}, we contrast this predictor with the one obtained with vector scaling and evaluate the loss information caused to due aggregation of predictions in terms of the Fisher information of our log-likelihood.
\todos{Ask how to pitch this? In general how to present this section?}

\begin{prop}\label{prop:calib}
Confusion matrix using a predictor $f$ in principle gives a per-label calibrated classifier on the source data. 
\end{prop}
The proof is in Appendix~\ref{sec:Appendixbgr}, which follows from the construction of confusion matrix and Definition~\ref{def:calib}.

\subsection{Finite sample error analysis} \label{subsec:finite}
% \todos[inline]{OK, so, all proofs go through for the positive support of $w^*$ and we can extrapolate for zero support with lemma-\ref{lemma:support}.}
 
We now analyze the MLLS estimators' convergence rates. For detailed proof from this section, we refer reader to Appendix \ref{sec:AppendixB}. 
Recall ${\widehat \w}$ denotes MLLS estimate~\eqref{optprob}. 
Let ${\w}^*$ denote the true shift. With consistency condition from section~\ref{subsec:consistency}, we assume that $\w^*$ is the population minimizer with the calibrated predictor $\fc =  \ProbS({ y= . | \widehat \f(\x) })$ .i.e. 
\begin{align}
\w^* = &\argmin_{w \in \W} - \E{\LL(\w; \fc )} \label{eq:MLLS_fc}
% &\quad \text{s.t.} \quad \sum_{y=1}^{k} w(y)\ps(y) = 1 \numberthis 
% &\quad \qquad \forall y \in \out \quad w(y) \ge 0 
\end{align}
 Our goal is to bound the finite sample error:  
\begin{equation}\label{eq:err}
    \Delta_n = ||\widehat \w - \w^*||_2 \le  \underbrace{||\widehat \w - \wc||_2}_{\RN{1}} +  \underbrace{||\wc - \w^*||_2}_{\RN{2}}  
\end{equation} 
where $ \wc$ is the finite sample estimation with the perfectly calibrated predictor $\fc$. We bound each error term on the RHS individually. Term-$\RN{1}$ denotes the estimation error due to finite sample re-calibration or inherent model misscalibration and term-$\RN{2}$ is the finite sample error with a perfectly calibrated model. 

% We use the following lemma
% % ~\ref{lemma:err_1} 
% to bound the error term-$\RN{2}$:  

\begin{lemma}[Error bound on term-$\RN{2}$]\label{lemma:err_1}
Assume the identifiability condition of lemma~\ref{lemma:identi-1} hold true and the predictor function  $\fc$ is bounded below at the non zero entries of $\w^*$ i.e. for all $\x$ such that $\pt(\x)>0$, we have $\sum_{y=1}^k \fc_y(\x) \w^*_y \ge \tau$ for some universal constant $\tau$. Let $\smin^{\fc}$ be the minimum eigenvalue of the Fisher information.  With probability at least $1-\delta$ we have,  
$$||\wc - \w^*||_2 \defeq \comp \left(\frac{1}{\smin^{\fc}}\sqrt{\frac{\log(\frac{4}{\delta})}{m}}\right)$$
\end{lemma}

\begin{proofsketch}

\end{proofsketch}


\begin{lemma}[Error bound on term-$\RN{1}$] \label{lemma:err_2}
Assume conditions from lemma \ref{lemma:err_1} hold true. Additionally assume the learnt predictor $\fh$ is also bounded below at the non zero entries of $\w^*$ i.e. for all $\x$ such that $\pt(\x)>0$, we have $\sum_{y=1}^k \fh_y(\x) \w^*_y \ge \tau$ for some universal constant $\tau$. Let $\smin^{\fh}$ be the minimum eigenvalue of the Fisher information with predictor $\fh$. With probability at least $1-\delta$ we have, 
\[
 || \wc - \widehat \w ||_2 \defeq \comp \left( \frac{1}{\sigma_{\min}^{\fh}}\Big(\sqrt{\frac{\log(\frac{4}{\delta})}{m}} +  \CE{\fh}||\w^*||_2 \Big) \right)
\]
\end{lemma}
\begin{proofsketch}

\end{proofsketch}

Depending on the degree of the miscalibration and method involved to calibrate $\fh$ we can bound the $\CE{\widehat \f}$. For example, if using vector scaling on a held out validation data from source for calibration, we can use lemma-\ref{lemma:platt} from Appendix \ref{sec:AppendixB} to bound the calibration error $\CE{\widehat \f}$ i.e. with standard regularity assumptions on model class $\G$ used for calibration we have with probability at least $1-\delta$,  
\begin{equation} \label{eq:platt}
  \CE{\fh} \le  \min_{\g \in \G} \CE{\g \circ \fh } + \sqrt{c\frac{\log(\frac{2}{\delta})}{n}}  
\end{equation}
  
\begin{theorem}[Error bounds] \label{thm:err}
Assume identifiability conditions of lemma \ref{lemma:identi-1} and assumption A.1 hold true. With probability at least $1-\delta$ we have, 
\begin{equation*}
\begin{split}
||\widehat \w - \w^*||_2  \defeq \comp \Bigg(\frac{1}{\smin^{\fc}}\sqrt{\frac{\log(\frac{4}{\delta})}{m}}  &+ \frac{1}{\sigma_{\min}^{\fh}}\Big(\sqrt{\frac{\log(\frac{4}{\delta})}{m}} \\ &+ \CE{\fh}||\w^*||_2 \Big) \Bigg)
\end{split}
\end{equation*}

\end{theorem}
The proof follows simply by combining above lemma's bounding the error terms $\RN{1}$ and $\RN{2}$ in \eqref{eq:err}. 

\todos[inline]{Remarks and takeaways from the above lemmas and theorem.}

\todos[inline]{Re-define the assumption from lemmas and justify that.}
To derive the finite sample bounds in lemma \ref{lemma:err_1} and \ref{lemma:err_2}, we make the following assumption: 

(A.1) \quad  


\textbf{Justification.} 
 
 
\todos[inline]{Explain what happens on the boundary} 

We begin this section by showing strong convexity of the log-likelihood. We need this condition for all our finite sample error analysis.

\begin{prop} \label{prop:strongconcave}
With the identifiability of the log-likelihood, the optimization problem~\eqref{optprob} is strongly convex.  
\end{prop}

The proof argument is detailed in Appendix-\ref{sec:AppendixB} the identifiability assumption. 


% \subsection{Generalization results} 
\todos{Majorly these will be from kamyar's paper which can be included for completeness.}


==> A Unified View of Label Shift Estimation (Neurips 2020)/sections/theory_new.tex <==
 \label{sec:finite}

We now analyze the performance of MLLS estimator. 
Even when $\w^*$ is the unique optimizer of \eqref{eq:mlls-main} for some calibrated predictor $\f$, assuming convex optimization can be done perfectly, there are still two sources of error preventing us from
exactly computing $\w^*$ in practice. 
First, we are optimizing a sample-based approximation \eqref{eq:mlls-sample} to the objective in expectation \eqref{eq:mlls-main}. 
We call this source of error \emph{finite-sample error}.  
Second, the predictor $\f$ we use may not be perfectly calibrated on the source distribution
% Edited %%%
% Perfect calibration might require full access
% to the source data distribution $p_s(\x, y)$,
% while 
% 
as 
we only have access to samples from source data distribution $p_s(\x, y)$. 
We call this source of error \emph{miscalibration error}.
We will first analyze how these two sources of errors affect the estimate of $\w^*$ separately 
and then give a general error bound that incorporates both.
All proofs are relegated to Appendix~\ref{sec:AppendixB}.
% For detailed proof from this section, we refer reader to Appendix \ref{sec:AppendixB}.

Before presenting our analysis, 
we introduce 
some notation and regularity assumptions. 
For any predictor $\f:\inpt\mapsto \Delta^{k-1}$, 
we define $\w_{\f}$ and $\widehat{\w}_{\f}$ as in~\eqref{eq:mlls-main} and~\eqref{eq:mlls-sample}.
%= \argmax_{w \in \W} \LL(\w; \f )$ 
%and
%$\widehat{\w}_{\f} = \argmax_{w \in \W} \LL_m(\w; \f )$ 
%% \begin{align}
%% \w_{\f} = \argmax_{w \in \W} \LL(\w; \f )  \label{eq:w-exp}
%% \end{align}
%% and
%% \begin{align}
%% \widehat{\w}_{\f} = \argmax_{w \in \W} \LL_m(\w; \f )  \label{eq:w-m}
%% \end{align}
%to be the maximizer for the expected and sample-based MLLS objective respectively. 
If $\f$ satisfies the conditions in Theorem~\ref{theorem:convergence} 
(calibration and linear independence) then we have that $\w_{\f} = \w^*$. 
Our goal is to bound $\norm{\widehat{\w}_{\f} - \w^*}$ 
for a given (possibly miscalibrated) predictor $\f$.
We now introduce a regularity condition:
% for a predictor $\f$:
\begin{condition}[Regularity condition for a predictor $\f$]
For any $\x$ within the support of $p_t(\x)$, i.e. $p_t(\x) > 0$, we have both $\f(\x)^T\w_{\f} \ge \tau$, $\f(\x)^T\w^* \ge \tau$ for some universal constant $\tau>0$.
\label{cond:tau}
% \vspace{-5pt}
\end{condition}
%XXXX editing here
% In general, Condition~\ref{cond:tau} is mild.
Condition~\ref{cond:tau} is mild if $\f$ is calibrated 
since in this case $\w_{\f} = \w^*$ 
is the maximizer of $\EE{t}{\log \f(\x)^T\w}$, and the condition is
satisfied if the expectation is finite. 
%so the expectation takes some finite value. 
Since $\f(\x)^T\w^*$ and $\f(\x)^T\w_{\f}$ are upper-bounded (they are the inner products of two vectors which sum to 1),
they also must be lower-bounded away from $0$
with arbitrarily high probability without any assumptions. 
%Further assuming no-tail for the distribution $p_t(\f(\x))$ 
%would be sufficient for the condition to hold.
For miscalibrated $\f$, a similar justification 
holds for assumption that $\f(\x)^T\w_{\f}$ is lower bounded. 
Turning our attention to the assumption that $\f(\x)^T\w^*$ is lower bounded, we note that 
it is sufficient if $\f$ is close (pointwise) to some calibrated predictor.
%, the condition is so not harsh 
%since $\f$ being similar to at least 
%one calibrated predictor is sufficient.
This in turn is a reasonable assumption 
on the actual predictor we use for MLLS in practice 
as it is post-hoc calibrated on source data samples.

% We discuss implications of this condition in detail in Section~\ref{subsec:disc_cond1}.  
%For the convenience of presenting our results, 
%we also introduce notation for the minimum eigenvalue 
%of the Hessian for the negative log-likelihood objective: 
Define $\sigma_{\f, \w}$ to be the minimum eigenvalue 
of the Hessian $- \nabla_{\w}^2 \LL(\w, \f)$. To state our results compactly
we use standard stochastic order notation (see, for instance,~\citep{van1996weak}). 
%Now we start to present our theoretical results.
% \paragraph{Finite-sample error.} 
We first bound the estimation error introduced
by only having finite samples from the target distribution in Lemma~\ref{lemma:bound-finite}. Next, we bound the estimation error introduced by having a miscalibrated $\f$ in Lemma~\ref{lemma:bound-calib}.

\begin{restatable}[]{relemma}{errone} \label{lemma:bound-finite}
% \begin{lemma}
For any predictor $\f$ that satisfies Condition~\ref{cond:tau}, we have % \begin{align*}
%\norm{\w_{\f} - \widehat{\w}_{\f}} = \comp_p \left( \frac{1}{\sigma_{\f}} \sqrt{\frac{1}{m}} \right) \,,
$\norm{\w_{\f} - \widehat{\w}_{\f}} \le \sigma_{\f, \w_{\f}}^{-1}  \comp_p \left(  m^{-1/2} \right).$
% \addeq\label{eq:bound-finite}
% \end{align*}
% \end{lemma}
% \vspace{-8pt}
\end{restatable}
% \vspace{-8pt}
\begin{restatable}[]{relemma}{errtwo}\label{lemma:bound-calib}
% \vspace{-5pt}
For any predictor $\f$ and any calibrated predictor $\f_c$ that satisfies Condition~\ref{cond:tau}, we have 
% \begin{align*}
%\norm{\w_{\f} - \widehat{\w}_{\f}} = \comp_p \left( \frac{1}{\sigma_{\f}} \sqrt{\frac{1}{m}} \right) \,,
$\norm{\w_{\f} - \w^*} \le  \sigma_{\f, \w^*}^{-1} \cdot C\cdot \EE{t}{\norm{\f - \f_c}} \,,$
% \addeq\label{eq:bound-calib}
% \end{align*}
for some constant $C$.

If we set $\f_c(\x) = p_s(y | \f(\x))$, 
which is a calibrated predictor (Proposition~\ref{prop:ltt-calib}), 
we can bound the error in terms of the calibration error of $\f$ on the source data \footnote{We present two upper bounds because the second is more interpretable while the first is tighter.}:
% \begin{align*}
%\norm{\w_{\f} - \widehat{\w}_{\f}} = \comp_p \left( \frac{1}{\sigma_{\f}} \sqrt{\frac{1}{m}} \right) \,,
$\norm{\w_{\f} - \w^*} \le \sigma_{\f, \w^*}^{-1} \cdot C\cdot\CE{\f} \,.$
% \addeq\label{eq:bound-calib-2}
% \end{align*}
% \vspace{-5pt}
\end{restatable}
% We formally prove these lemmas in Appendix~\ref{sec:AppendixB}.
% but give a proof sketch here.  
% Lemmas~\ref{lemma:bound-finite} and \ref{lemma:bound-calib} 
% bound the difference between the optimizers of two different functions. 
% The proof starts with a second-order Taylor expansion 
% of one function around the optimum of the other function.
% Using this Taylor expansion, we relate the estimation error 
% to the difference between the gradient 
% of two functions evaluated at the same point, e.g.,
% $\norm{\nabla_{\w} \LL_m(\w_{\f},\f) - \nabla_{\w} \LL(\w_{\f},\f)}$ for
% Lemma~\ref{lemma:bound-finite} and $\norm{\nabla_{\w} \LL(\w^*,\f) - \nabla_{\w} \LL(\w^*,\f_c)}$ 
% for Lemma~\ref{lemma:bound-calib}. 
% For Lemma~\ref{lemma:bound-finite}, 
% we then use a concentration inequality 
% to bound the difference in gradients, 
% while for Lemma~\ref{lemma:bound-calib}, 
% we exploit the Lipschitzness of the gradient
% to relate the difference in gradients 
% to the difference in function values.
% 
% \paragraph{Total estimation error.} Now 
% \textcolor{red}{
Note that since $p_s(y)>0$ for all $y$, we can upper-bound the error 
in Lemma~\ref{lemma:bound-calib} with calibration error 
on the source data.
% which is an observable quantity.
% }
We combine the two sources of error to bound the estimation error $\norm{\widehat{\w}_{\f} - \w^*}$:
\begin{restatable}[]{rethm}{main-error-bound}\label{theorem:main-error-bound}
% \begin{theorem} \label{theorem:MLLS_err}
For any predictor $\f$ that satisfies Condition~\ref{cond:tau}, we have
\begin{align*}
\norm{\widehat{\w}_{\f} - \w^*} \le \sigma_{\f, \w_{\f}}^{-1} \comp_p \left(  m^{-1/2} \right) + C\cdot \sigma_{\f, \w^*}^{-1} \CE{\f} \,. \addeq\label{eq:bound-main} 
\end{align*}
\end{restatable}
% \vspace{-5pt}
The estimation error of MLLS can be decomposed into 
(i) finite-sample error, which decays at a rate of $m^{-1/2}$;
and (ii) the calibration error of the predictor that we use.
% Theorem~\ref{theorem:main-error-bound} shows that the estimation error of MLLS can be decomposed into (i) finite-sample error, which decays at a rate of $m^{-1/2}$ and (ii) the calibration error of the predictor that we use.
The proof is a direct combination of Lemma~\ref{lemma:bound-finite} 
and Lemma~\ref{lemma:bound-calib} applied to the same $\f$ with the following error decomposition:
\begin{align*}
\norm{\widehat{\w}_{\f} - \w^*} \le  \underbrace{ \norm{\w_{\f} - \widehat{\w}_{\f}}}_{\textrm{finite-sample}} +  \underbrace{\norm{\w_{\f} - \w^*}}_{\textrm{miscalibration}} \,.
% \vspace{-50pt}    
\end{align*}
Theorem~\ref{theorem:main-error-bound} shows that 
the estimation error depends inversely 
on the minimum eigenvalue of the Hessian 
at two different points $\w_{\f}$ and $\w^*$. 
One can unify these two eigenvalues 
as a single quantity $\sigma_{\f}$, the minimum eigenvalue $\EE{t}{\f(\x)\f(\x)^T}$. We formalize this observation 
% in Proposition~\ref{prop:eigen} 
in Appendix~\ref{sec:AppendixB}. 
% \todos{Shifted this prop to Appendix}

% by the following observation:

% \vspace{-8pt}
% Proposition~\ref{prop:eigen} shows that we can combine 
% the two eigenvalues in Theorem~\ref{theorem:main-error-bound} 
% to a single $\sigma_{\f}$ and this relaxation is tight up to the constant factors.
% described in~\eqref{eq:eigen-relax}.


% Depending on the degree of the miscalibration and method involved for post-hoc calibration, we can bound $\CE{\f}$. For example, if a predictor model $\f^\prime$ was calibrated using vector scaling~\citep{guo2017calibration},
% % on a held out validation data from source for 
% % post-hoc  of $\f^\prime$,
% we can use Lemma~\ref{lemma:platt} from Appendix~\ref{sec:AppendixB} to bound the calibration error of $\f$. Under standard regularity assumptions on model class $\G$ used for vector scaling we have,



If we use the \emph{post-hoc calibration} procedure
(as discussed in Section~\ref{sec:pre} and~\ref{sec:MLLs_alg}) to calibrate a blackbox predictor $\smash{\widehat{\f}}$, 
we can obtain a bound on the calibration error of $\f$. In more detail, suppose that the class $\G$ 
used for calibration satisfies standard regularity conditions (injectivity, Lipschitz-continuity, twice differentiability, non-singular Hessian).
% described in detail in Theorem 5.23 of \citet{stein1981estimation}. 
We have the following lemma:  
\begin{restatable}[]{relemma}{ce}\label{lemma:ce}
% \begin{lemma}
Let $\f = \g \circ \widehat{\f}$ be the predictor after post-hoc calibration 
with squared loss $l$ and $\g$ belongs to a function class $\G$ 
that satisfies the standard regularity conditions, we have 
\begin{align}\label{eq:platt}
\CE{\f} \le  \min_{\g \in \G} \CE{\g \circ \widehat{\f} } + \comp_p\left( n^{-1/2}\right) \,. 
\end{align}
\end{restatable}
%
% \vspace{-8pt}

This result is similar to Theorem 4.1~\cite{kumar2019verified}. 
For a model class $\G$ that is rich enough to contain a function $\g \in \G$ 
that achieves zero calibration error, i.e.,
$\min_{\g \in \G} \CE{\g \circ \widehat{\f} } = 0$, 
%\footnote{Note, here we are not assuming we recover this model $\g$ with finite validation samples.}. 
then we obtain an estimation error bound for MLLS 
of $\sigma_{\f}^{-1} \cdot\comp_p \left(  m^{-1/2} +  n^{-1/2}\right)$. 
This bound is similar to rate of RLLS and BBSE,
where instead of $\sigma_{\f}$ they have minimum eigenvalue of the confusion matrix.
% \textcolor{red}{Although these constants here are not directly comparable }

% \textcolor{red}{
% Addressing question 3
% answer the third question from
% 
% 

% 
% 
The estimation error bound explains the efficiency of MLLS.
% over BBSE.
Informally, the error of MLLS depends inversely
on the minimum eigenvalue of the Hessian of the likelihood $\sigma_{\f}$.
When we apply coarse calibration via the confusion matrix (in MLLS-CM),
we only decrease the value of $\sigma_{\f}$.
Coarse calibration throws away information~\citep{kuleshov2015calibrated} and thus results 
in greater estimation error for MLLS. 
% 
% (Section~\ref{subsec:MLLS}), 
% we point to
% via the finite sample estimation bound.
In Section~\ref{sec:exp}, we empricially show that MLLS-CM's performance
is similar to that of BBSE. 
Moreover, on a synthetic Gaussian mixture model, 
we show that the minimum eigenvalue of the Hessian obtained 
using confusion matrix calibration is smaller than the minimum eigenvalue obtained with more granular calibration. 
Our analysis and observations together suggest MLLS's superior performance than BBSE (or RLLS)
is due to the granular calibration but not 
due to the difference in the optimization objective. 
% 
% We discuss a detailed discussion, including
% In Appendix~\ref{subsec:err_discuss}, we include more discussions to confusion matrix approaches. 
% } 
% \todos{Comment on the relation?}

Finally, we want to highlight one minor point regarding applicability of our result.
%for completeness. 
If $\f$ is calibrated, Theorem~\ref{theorem:main-error-bound},
together with Proposition~\ref{prop:eigen} (in Appendix~\ref{sec:AppendixB}),
implies that MLLS is consistent if $\EE{t}{\f(\x)\f(\x)^T}$ is invertible. 
Compared to the consistency condition in Theorem~\ref{theorem:mlls} 
that $\EE{s}{\f(\x)\f(\x)^T}$ is invertible 
(together with Proposition~\ref{prop:equiv-cond}), 
these two conditions are the same if the likelihood ratio $p_t(\f(\x)) / p_s(\f(\x))$ is lower-bounded. 
This is true if all entries in $\w^*$ are non-zero. 
Even if $\w^*$ contains non-zero entries, 
the two conditions are still the same if there exists some $\w^*_y > 0$ 
such that $p(\f(\x)|y)$ covers the full support of $p_s(\f(\x))$. 
In general however, the invertibility of $\EE{t}{\f(\x)\f(\x)^T}$ 
is a stronger requirement than the invertibility of $\EE{s}{\f(\x)\f(\x)^T}$.
We leave further investigation of this gap for future work. 


%\section{Finite Sample Error Bounds}
%\subfile{sections/finite.tex}

% \subsection{Algorithm}


==> A Unified View of Label Shift Estimation (Neurips 2020)/sections/unify.tex <==
\newcommand{\ltt}{\mathcal{Z}}
\newcommand{\W}{\mathcal{W}}
\newcommand{\z}{z}
% Given these preliminaries,
% 
% We can now provide a unified view of label shift estimation 
% that leverage off-the-shelf classifier 
We now present a unified view that subsumes MLLS and BBSE
% 
% 
% as finding latent parameters of a generative model
% that match the target data distribution,
% 
% in some latent space. 
and demonstrate how each is instantiated under this framework. 
% In this section,
We also establish identifiability and consistency conditions for MLLS, 
% Throughout this section, 
% For now, we assume knowledge of the true $p_s(\x, y)$ and $p_t(\x)$,
deferring a treatment of finite-sample issues to Section \ref{sec:finite}. 
For convenience, throughout Sections 3 and 4, 
we use the term \emph{calibration} exclusively 
to refer to canonical calibration 
(Definition~\ref{def:calib}) on the source data. 
We relegate all technical proofs to Appendix~\ref{sec:AppendixA}. 

\vspace{-5pt}
\subsection{A Unified Distribution Matching View}
\vspace{-5pt}

To start, we introduce a \emph{generalized} distribution
matching approach for estimating $\w$. 
Under label shift, for any (possibly randomized) mapping 
from $\inpt$ to $\ltt$, we have that
$p_s(\z|y)=p_t(\z|y)$ since,
% \begin{align*}
$\smash{p_s(\z|y)=p_t(\z|y)=\int_{\mathcal{X}} \, p(\z|\x)p(\x|y)dx.}$
% \end{align*}
%
%
%given any fixed conditional distribution $p(\z|\x)$ 
%from the input space $\inpt$ 
%to another space $\ltt$, 
%we have $p_s(\z|y)=p_t(\z|y)$ as $p_s(\z|y)=p_t(\z|y)=\int \, p(\z|\x)p(\x|y)dx$. 
Throughout the paper, we use the notation $p(\z|y)$
to represent either $p_s(\z|y)$ or $p_t(\z|y)$ (which are identical). 
We now define a family of distributions over 
% the latent space 
$\ltt$ parameterized by $\w\in \W$ as
% \vspace{-5pt}
\begin{align}
\label{eqn:pwdef}
p_{\w}(\z) = \sum\nolimits_{y=1}^k p(\z|y)p_s(y)\w_y = \sum\nolimits_{y=1}^k p_s(\z, y)\w_y, 
% \vspace{-5pt}
\end{align}
% $p_{\w}(\z) = \sum_{y=1}^k p(\z|y)p_s(y)\w_y = \sum_{y=1}^k p_s(\z, y)\w_y\,,$ 
where $\smash{\W = \{ \w \; |\; \forall y \,,  w_y \ge 0 \text{ and } \sum_{y=1}^{k} w_y \ps(y) = 1 \}}$.     
When 
% $\w$ is the true label distribution ratio, i.e. 
$\w=\w^*$, we have that $p_{\w}(\z) = p_t(\z)$. For fixed $p(\z|\x)$, $p_t(\z)$ and $p_s(\z, y)$ are known because $p_t(\x)$ and $p_s(\x, y)$ are known. 
So one potential strategy to estimate $\w^*$ is 
to find a weight vector $\w$ such that 
% \vspace{-5pt}
\begin{align*}
\sum\nolimits_{y=1}^k p_s(\z, y)\w_y = p_t(\z) ~~~~ \forall \z\in \ltt \,. \addeq\label{eq:distr-match}
% \vspace{-5pt}
\end{align*}
% \vspace{-5pt}
At least one such weight vector $\w$ must exist as $\w^*$ satisfies \eqref{eq:distr-match}. 
% The following Lemma characterizes 
We now characterize
% the identifiability of this approach, i.e.,
conditions under which the weight vector $\w$ satisfying \eqref{eq:distr-match} is unique:
% \begin{restatable}[Identifiability]{relemma}{identifiability}
% % \begin{lemma}[]
% If the set of distributions $\{p(\z|y)\,:\, y=1,...,k\}$ are linearly independent \footnote{For continuous case, with linear independence we mean that we should not loose linear independence by removing any zero measure set from our domain $\ltt$, i.e., there does not exist $\vv \ne 0$ such that $\int \abs{\sum_y p(\z|y) v_y} d\z = 0$ }\todos{For continuous case, this should be true by definition of smoothness and continuity on the density function p(z|y).},
% then for any $\w$ that satisfies \eqref{eq:distr-match}, we must have $\w=\w^*$. 
% This condition is also necessary in general: 
% if the linear independence does not hold 
% then there exists a problem instance where 
% we have $\w, \w^* \in \W$ satisfying \eqref{eq:distr-match} while $\w \ne \w^*$.
% \label{lemma:identi-1}
% % \end{lemma}
% \end{restatable}

\begin{restatable}[Identifiability]{relemma}{identifiability}
\label{lemma:identi-1}
% \begin{lemma}[]
If the set of distributions $\{p(\z|y)\,:\, y=1,...,k\}$ are linearly independent,
then for any $\w$ that satisfies \eqref{eq:distr-match}, we must have $\w=\w^*$. 
This condition is also necessary in general: 
if the linear independence does not hold 
then there exists a problem instance where 
we have $\w, \w^* \in \W$ satisfying \eqref{eq:distr-match} while $\w \ne \w^*$. 
% \end{lemma}
% \vspace{-5pt}
\end{restatable}


% \todos{Add this as prop?}
Lemma~\ref{lemma:identi-1} follows from the fact 
that \eqref{eq:distr-match} is a linear system 
% where the 
with at least one solution $\w^*$. This solution is 
% Then uniqueness of the solution to a linear system applies: 
% The solution to \eqref{eq:distr-match}
unique when $p_s(\z, y)$ is of rank $k$.
% which is 
% Assuming that $p_s(y)>0$ for all $y$ (as we have throughout this paper),
% this is equivalent to the linear independence condition. 
The linear independence condition in Lemma~\ref{lemma:identi-1}, in general, is sufficient for identifiability of discrete $\ltt$. 
% 
% However, for continuous $\ltt$, we impose a \emph{strict linear independence}\footnote{We define and discuss this more in Appendix~\ref{}}.  
% 
However, for continuous $\ltt$, the linear dependence condition has the undesirable property of being sensitive to changes on sets of measure zero.
By changing a collection of linearly dependent distributions on a set of measure zero, we can make them linearly independent.
As a consequence, we impose a \emph{stronger} notion of identifiability i.e., the set of distributions $\{p(\z|y)\,:\, y=1,...,k\}$ are such that there does not exist $\vv \ne 0$ for which 
% \begin{align*}
    $\smash{\int_{\ltt} \lvert{\sum_y p(\z|y) v_y}\rvert d\z = 0.}$ 
    % \numberthis \label{eq:strong_ind}
% \end{align*} 
% \todos{For continuous case, this should be true by definition of smoothness and continuity on the density function p(z|y).}
We refer 
% to \eqref{eq:strong_ind} 
this condition as \emph{strict linear independence}. 
% of the set of distributions $\{p(\z|y)\,:\, y=1,...,k\}$.   

In generalized distribution matching, one can set $p(\z|\x)$ to be the Dirac delta function 
at $\delta_{\x}$\footnote{For simplicity we will use $\z=\x$ 
to denote that $p(\z|\x)=\delta_{\x}$.}
such that $\ltt$ is the same space as $\inpt$, 
which leads to solving \eqref{eq:distr-match} with $\z$ replaced by $\x$. 
In practice where $\inpt$ is high-dimensional and/or continuous,
% while we only have finite number of samples from $p_s(\x, y)$ and $p_t(\x)$, 
approximating the solution to \eqref{eq:distr-match} from finite samples
can be hard when choosing $\z=\x$. 
% The motivation for generalizing this 
% We generalize 
Our motivation for generalizing
distribution matching from $\inpt$ to 
% some latent space
$\ltt$ is that the solution to \eqref{eq:distr-match} 
can be better approximated using finite samples 
when $\ltt$ is chosen carefully.
% by choosing $p(\z|\x)$ appropriately. 
Under this framework, the design of a label shift 
estimation algorithm can be decomposed into two parts: 
(i) the choice of $p(\z|\x)$ and
(ii) how to approximate the solution to \eqref{eq:distr-match}. 
Later on, we consider how these design choices 
may affect label shift estimation procedures in practice.

\vspace{-7pt}
\subsection{The Confusion Matrix Approach} 
\vspace{-5pt}

If $\ltt$ is a discrete space, one can first estimate 
$p_s(\z, y) \in \Real^{|\ltt|\times k}$ and 
$p_t(\z) \in \Real$, and then subsequently attempt 
to solve \eqref{eq:distr-match}.
Confusion matrix approaches use $\ltt = \out$, 
and construct $p(\z|\x)$ using a black box predictor $\widehat{\f}$. 
There are two common choices to construct the confusion matrix:
% 
% \begin{enumerate}[noitemsep,topsep=5pt]
(i) The soft confusion matrix approach:
We set $p(\z|\x) := \widehat{\f}(\x) \in \Delta^{k-1}$. 
We then define a random variable $\widehat{y} \sim \widehat{\f}(\x)$ for each $\x$. 
Then we construct $p_s(\z, y) = p_s(\widehat{y}, y)$ and $p_t(\z)=p_t(\widehat{y})$. 
% 
(ii) The hard confusion matrix approach: Here we set $p(\z|\x)=\delta_{\argmax\widehat{\f}(\x)}$. 
We then define a random variable $\widehat{y} =\argmax \widehat{\f}(\x)$ for each $\x$. 
Then again we have $p_s(\z, y) = p_s(\widehat{y}, y)$ and $p_t(\z)=p_t(\widehat{y})$. 
% \end{enumerate}

Since $p_s(\z, y)$ is a square matrix, 
the identifiability condition becomes 
the invertibility of the confusion matrix. 
% Given the estimated confusion matrix, one can find $\w$ by inverting the confusion matrix (BBSE) or minimizing the difference (e.g. L2) between the vectors on the two sides of \eqref{eq:distr-match}. 
Given an estimated confusion matrix, one can find $\w$ by inverting the confusion matrix (BBSE) or minimizing
some distance 
%the Maximum Mean Discrepancy (MMD) 
between the vectors on the two sides of \eqref{eq:distr-match}. 

% % \todoy{Move intro to CM from sec 2 to here?}
% If $\ltt$ is a discrete space, one can first estimate 
% $p_s(\z, y) \in \Real^{|\ltt|\times k}$ and 
% $p_t(\z) \in \Real$, and then 
% % subsequently 
% % attempt 
% % to 
% solve \eqref{eq:distr-match}.
% In this framework, confusion matrix approaches use $\ltt = \out$, 
% and construct $p(\z|\x)$ using a black box predictor $\smash{\widehat{\f}}$. 
% % \textcolor{red}{
% In Appendix~\ref{subsec:construction}, we discuss the estimation 
% of $p_s(\z,y)$ from the hard and soft confusion matrix.
% % }  
% %
% Since $p_s(\z, y)$ is a square matrix, 
% the identifiability condition becomes 
% the invertibility of the confusion matrix. 
% % Given the estimated confusion matrix, one can find $\w$ by inverting the confusion matrix (BBSE) or minimizing the difference (e.g. L2) between the vectors on the two sides of \eqref{eq:distr-match}. 
% Given an estimated confusion matrix, one can find $\w$ by inverting the confusion matrix (BBSE) or minimizing
% some distance 
% %the Maximum Mean Discrepancy (MMD) 
% between the vectors on the two sides of \eqref{eq:distr-match}. 
% \todos{Maybe we can say this would be MMD and RLLS is same as this with an extra regularization term} 
%In Appendix~\ref{apx:IPM}, we show that minimizing L2 distance between vectors on the two side of \eqref{eq:distr-match}
%is same as minimizing MMD with $\ltt = \out$. 

\vspace{-7pt}
\subsection{Maximum Likelihood Label Shift Estimation} \label{subsec:MLLS}
\vspace{-5pt}

When $\ltt$ is a continuous space, 
the set of equations in \eqref{eq:distr-match} indexed by $\ltt$ is intractable. 
% So it is desirable to have 
In this case, 
%we desire a sample-based method 
%to solve \eqref{eq:distr-match} approximately. 
% This is doable by 
one possibility is to 
%solve \eqref{eq:distr-match} 
find a weight vector $\widetilde{\w}$
by minimizing the KL-divergence
% $\mathrm{KL}(p_t(\z), p_{\w}(\z)) = \EE{\z\sim p_t(\z)}{\log p_t(\z) / p_{\w}(\z)}$, 
$\mathrm{KL}(p_t(\z), p_{\w}(\z)) = \EE{t}{\log p_t(\z) / p_{\w}(\z)}$, for 
$p_{\w}$ defined in~\eqref{eqn:pwdef}.
This is equivalent to maximizing the population log-likelihood:
% \begin{align*}
% \max_{w \in \W} \EE{\z\sim p_t(\z)}{ \log p_{\w}(\z)} \,.\addeq\label{eq:mle-z}
$\smash{\widetilde{w} := \argmax_{w \in \W} \EE{t}{ \log p_{\w}(\z)}}\,.$
% \addeq\label{eq:mle-z}
% \end{align*}
% One can further show that 
% \allowdisplaybreaks
% \begin{align*}
% & \EE{\z\sim p_t(\z)}{ \log p_{\w}(\z)}
% = \EE{\z\sim p_t(\z)}{ \log \sum_{y=1}^k p_s(\z, y)\w_y} \\
% & = \EE{\z\sim p_t(\z)}{ \log \sum_{y=1}^k p_s(y|\z) p_s(\z) \w_y} \\
% & = \EE{\z\sim p_t(\z)}{ \log \sum_{y=1}^k p_s(y|\z)  \w_y} + \EE{\z\sim p_t(\z)}{p_s(\z)} \,.
% \end{align*}
% Therefore the objective \eqref{eq:mle-z} is equivalent to
% \begin{align*}
% \max_{w \in \W} \EE{\z\sim p_t(\z)}{ \log \sum_{y=1}^k p_s(y|\z)  \w_y} \,.\addeq\label{eq:mlls-z}
% \end{align*}
One can further show that 
\allowdisplaybreaks
% \begin{align*}
$\EE{t}{ \log p_{\w}(\z)}
= \mathbb{E}_{t}[\log \sum_{y=1}^k p_s(\z, y)\w_y]  = \mathbb{E}_{t}[ \log \sum_{y=1}^k p_s(y|\z) p_s(\z) \w_y]
= \mathbb{E}_{t}[ \log \sum_{y=1}^k p_s(y|\z)  \w_y] + \EE{t}{\log p_s(\z)}.$
% \end{align*}
Therefore we can equivalently define:
% \vspace{-5pt}
\begin{align*}
\widetilde{w} := \argmax_{w \in \W} \mathbb{E}_t \Big[ \log \sum\nolimits_{y=1}^k p_s(y|\z)  \w_y\Big] \,.\addeq\label{eq:mlls-z}
% \vspace{-5pt}
\end{align*}
% \vspace{-5pt}
%%% Added from next section
% The above optimization 
% This objective is concave and bounded from above.
This yields a straightforward convex optimization problem
whose objective is bounded from below
%\todos{Correct the term}
% as shown in 
\citep{alexandari2019adapting, du2014semi}. 
% \todos{From wiki, the problem of maximizing a concave function over a convex set is often referred to as a convex optimization problem.}
% Under the assumption of non-zero support of source labels, i.e., 
% the assumption that for all $y \in \out$ $~ \ps(y) = c > 0$ , 
% the likelihood objective is also bounded from above by $-\log(c)$.  
% \todos{I removed the proposition and saved the lines for proof argument}
% In Appendix~\ref{sec:AppendixB}, we also show that the optimization problem is also self concordant (Proposition~\ref{prop:sc}). 
% \begin{restatable}[\citet{alexandari2019adapting}]{reprop}{convex}
% \label{prop:convex}
% % \begin{prop} 
% Optimization problem \eqref{eq:mlls-z} is convex. 
% % \end{prop}
% \end{restatable} 
% The proof argument follows simply:
% Our objective is to minimize the negative log 
% of a convex combination of a linear function in parameters. 
% The minimization is over a convex region
% %i.e. a simplex of dimensions $k-1$
% and thus the problem is convex.
% %%%
Assuming access to labeled source data 
and unlabeled target data,
%$p_s(y|\z)$ and samples from $p_t^{\ltt}$ \footnote{We use this notation to denote samples from the target distribution over $\ltt$.}, 
one can maximize 
% a sample-based approximation to 
the empirical counterpart of the objective in~\eqref{eq:mlls-z},
% tractably, 
using either EM or an alternative iterative optimization scheme.
\citet{saerens2002adjusting} derived an EM algorithm to maximize the objective \eqref{eq:mlls-z} when $\z=\x$, 
assuming access to $p_s(y|\x)$. 
% When we don't know 
Absent knowledge of the ground truth $p_s(y|\x)$, 
% is not accessible, 
% one 
we can plug in any approximate predictor $\f$ 
and optimize the following objective:
% \begin{align*}
% \max_{w \in \W} \EE{t}{ \log \f(\x)^T  \w} \,.\addeq\label{eq:mlls-main}
% \end{align*}
% \vspace{-5pt}
\begin{align*}
w_f := \argmax_{w \in \W} \LL(\w,\f) := \argmax_{w \in \W} \EE{t}{ \log \f(\x)^T  \w} \,.\addeq\label{eq:mlls-main}
\vspace{-5pt}
\end{align*}
%We name \eqref{eq:mlls-main} as \textbf{Maximum Likelihood Label Shift (MLLS)} estimation.
%as it tries to maximize the log-likelihood $\EE{t}{ \log p_{\w}(\x)}$ approximately. 
% (MLLS)
% 
% 
% We name \eqref{eq:mlls-main} 
% \textbf{maximum likelihood label shift estimation} 
% because it maximizes the empirical approximation to  log-likelihood $\EE{t}{ \log p_{\w}(\x)}$. 
% 
%We denote the population log-likelihood $\EE{t}{ \log \f(\x)^T  \w}$ as $\LL(\w, \f)$. 
In practice, $\f$ is fit 
from a finite %number of
sample drawn from $p_s(\x, y)$ 
and standard machine learning methods
often produce uncalibrated predictors.
% that are uncalibrated.
% predictor $\f$ can be biased and uncalibrated.  
% the quality of $\f$ 
% \todos{Maybe we can re-write this statement? I got the idea but I think we can improve this sentence} 
% (how close it is to $p_s(\x, y)$) differs from task to task. 
While BBSE and RLLS are provably consistent 
whenever the predictor $\f$ yields an invertible confusion matrix, 
% 
% i.e. the estimated $\w$ can get arbitrarily closer to $\w^*$ as the number of samples increases,
% 
% Unlike BBSE where the estimator of $\w^*$ is \todos{provably} consistent even when $\f$ is a blackbox predictor, i.e. the estimated $\w$ can get arbitrarily closer to $\w^*$ as the number of samples increases, 
% for MLLS 
% it is unclear whether the performance can still be guaranteed when $\f$ differs from $p_s(y|\x)$.
to our knowledge, no prior works have established sufficient conditions 
to guarantee  MLLS' consistency when $\f$ differs from $p_s(y|\x)$.
% Intuitively, there should be an intrinsic error in estimation of $\w^*$ due to the difference between $\f$ and $p_s(y|\x)$.

It is intuitive that for some values of $\f \neq p_s(y|\x)$, MLLS will yield inconsistent estimates. 
Supplying empirical evidence, \citet{alexandari2019adapting} show that MLLS performs poorly 
when $\f$ is a vanilla neural network predictor learned from data.
However, \citet{alexandari2019adapting} also show that
in combination with a particular post-hoc calibration technique,
MLLS achieves low error, significantly outperforming BBSE and RLLS. 
As the calibration error is not a distance metric between $\f$ and $p_s(y|\x)$ 
(zero calibration error does not indicate $\f=p_s(y|\x)$),
a calibrated predictor $\f$ may still be substantially different from $p_s(y|\x)$. 
Some natural questions then arise: 

\begin{enumerate}[noitemsep,topsep=0pt]
\setlength\itemsep{4pt}
\item \emph{Why does calibration improve MLLS so dramatically?}
\item \emph{Is calibration necessary or sufficient to ensure the consistency of MLLS?}
\item \emph{What accounts for the comparative efficiency of MLLS 
% with BCTS calibration 
over BBSE?} (Addressed in Section~\ref{sec:finite})
\end{enumerate}

% And why does calibrated 
%  even better than a consistent estimator while there is no guarantee on the gap between 
% the objective we are optimizing (\eqref{eq:mlls-main} with calibrated $\f$) and the ground truth objective (\eqref{eq:mlls-z} with $\z=\x$)?}

% \emph{Why does calibration makes MLLS even better than a consistent estimator while there is no guarantee on the gap between 
% the objective we are optimizing (\eqref{eq:mlls-main} with calibrated $\f$) and the ground truth objective (\eqref{eq:mlls-z} with $\z=\x$)?}

% \noindent \textcolor{red}{We answer the third question in Section~\ref{sec:finite}.} 
To address the first two questions, 
we make the following observations. 
Suppose we define $z$ (for each $x$) with distribution 
$p(\z| \x) := \delta_{\f(\x)}$, for some calibrated predictor $f$. 
Then, because $f$ is calibrated,
it holds that $p_s(y | \z) = f(x)$.
% 
% Maybe add this as proposition? :p
% 
% In other words, 
Note that in general,
the MLLS objective~\eqref{eq:mlls-main} can 
differ from~\eqref{eq:mlls-z}. 
However, when $p(\z| \x) := \delta_{\f(\x)}$, 
the two objectives are identical.
%\emph{Even though a calibrated predictor $\f$ is not sufficient to
%make the MLLS objective \eqref{eq:mlls-main} the same as \eqref{eq:mlls-z} with $\z=\x$,
%calibration of $\f$ is sufficient to make \eqref{eq:mlls-main}
%the same as \eqref{eq:mlls-z} with some other $p(\z|\x)$. 
%}
% The following Lemma formally states this observation:
We can formalize this as follows:
\begin{restatable}[]{relemma}{calibobj}
% \begin{lemma}
If $\f$ is calibrated, then the two objectives~\eqref{eq:mlls-z} and~\eqref{eq:mlls-main}
are identical when $\ltt$ is chosen as $\Delta^{k-1}$ and \mbox{$p(\z|\x)$} is defined to be {$\delta_{\f(\x)}$}.
\label{lemma:calib}
% \end{lemma}
% \vspace{-5pt}
\end{restatable}
Lemma~\ref{lemma:calib} follows from changing 
the variable of expectation in \eqref{eq:mlls-main} from $\x$ to $\f(\x)$ 
and applying $\f(\x)=p_s(y|\f(\x))$ (definition of calibration). 
It shows that MLLS with a calibrated predictor on the input space $\inpt$ 
is in fact equivalent to performing 
distribution matching in the space $\ltt$.
Building on this observation, we now state our % main 
population-level consistency theorem for MLLS:

\begin{restatable}[Population consistency of MLLS]{rethm}{consistency}
% \begin{theorem}[]
If a predictor $\f: \inpt \mapsto \Delta^{k-1}$ is calibrated and the distributions 
$\{p(\f(\x)|y)\,:\,y=1,\ldots,k\}$ are strictly linearly independent, 
then $\w^*$ is the unique maximizer of the MLLS objective~\eqref{eq:mlls-main}.
\label{theorem:mlls}
% \end{theorem}
% \vspace{-5pt}
\end{restatable}

We now turn our attention to establishing consistency of the sample-based estimator.
% in Theorem~\ref{theorem:convergence}.
Let \allowdisplaybreaks{$\x_1, \x_2, \ldots, \x_m \stackrel{iid}{\sim} \pt(x)$}. 
The finite sample objective for MLLS can be written as
% \vspace{-5pt}
\begin{align*}
\widehat{w}_f := \argmax_{w \in \W} \frac{1}{m} \sum\nolimits_{i=1}^m \log \f(\x_i)^T  \w := \argmax_{w \in \W} \LL_m(\w, \f) \,.\addeq\label{eq:mlls-sample}
\end{align*}
% \vspace{-5pt}
\begin{restatable}[Consistency of MLLS]{rethm}{convergence}
% \begin{corollary}
\label{theorem:convergence}
If $\f$ satisfies the conditions in Theorem~\ref{theorem:mlls}, then $\widehat{w}_f$ in~\eqref{eq:mlls-sample} converges to $\w^*$ almost surely. 
% \vspace{-5pt}
% \end{corollary}
\end{restatable}



% The proof of Theorem~\ref{theorem:mlls} is a direct combination of Lemma~\ref{lemma:identi-1}, 
% Lemma~\ref{lemma:calib},
% and an elementary property of the KL-divergence. 
The main idea of the proof of Theorem~\ref{theorem:convergence} is to derive a metric entropy bound on the class of functions $\mathcal{G} = \left\{ (f^Tw)/(f^Tw + f^Tw^*) | w\in \mathcal{W} \right\}$ to prove Hellinger consistency (Theorem 4.6~\citep{geer2000empirical}). 
The consistency of MLLS 
relies on the linear independence of
the collection of distributions $\{p(\f(\x)|y)\,:\,y=1,\ldots,k\}$. 
The following result develops several alternative equivalent characterizations 
of this linear independence condition. 

% We can also state the linear independence condition in other ways:
\begin{restatable}[]{reprop}{equivalent} 
\label{prop:equiv-cond}
For a calibrated predictor $\f$, the following statements are equivalent:
\begin{enumerate}[itemsep=-.5ex,topsep=0pt,label=(\arabic*)]
% \setlength\itemsep{4pt}
\item $\{p(\f(\x)|y)\,:\,y=1,\ldots,k\}$ are strictly linearly independent.
% \item $\EE{\x\sim p_s(\x)}{\f(\x)\f(\x)^T}$ is invertible.
\item $\EE{s}{\f(\x)\f(\x)^T}$ is invertible.
\item The soft confusion matrix of $\f$ is invertible.
\end{enumerate}
% \vspace{-5pt}
\end{restatable}

% \textcolor{red}{
Proposition~\ref{prop:equiv-cond} shows that with a calibrated predictor,
the invertibility condition as required by BBSE (or RLLS)
is exactly the same as the linear independence condition 
required for MLLS's consistency.
% }
% We now turn our discussion to that. 
% \todoy[inline]{we need to check the correctness then polish the proof sketch} 

% We need uniform convergence on the log-likelihood to prove Corollary~\ref{corollary:convergence} . Once uniform convergence is established the proof for convergence in probability follows trivially from Corollary $\RN{2}.2$~\cite{andersen1982cox} and Theorem~\ref{theorem:mlls}. 
% For proving uniform convergence, we use Theorem $\RN{2}.1$~\cite{andersen1982cox} for $\w^*$ which lies in the interior of $\W$. For points lying on the boundary, we take a union over a finite sets for which we have uniform convergence to complete the proof for uniform convergence over the whole set $\W$. 
% We detail this argument in the appendix \ref{sec:AppendixA}.  

% ~\cite{lecturenotes}

% \begin{lemma}[Uniform Convergence~\cite{andersen1982cox}] \label{lemma:uc}
% Suppose a sequence of convex function $\LL_m(\w, \f)$ converges in probability to $\LL(\w, \f)$ for $w$ in an open set $\mathcal{W}$, then $\sup_{\mathcal{W}^\prime} \abs{\LL_m(\w, \f) - \LL(\w, \f)}$ goes to zero in probability on every compact subset $\mathcal{W}^\prime$ of $\mathcal{W}$.     
% \end{lemma}


% \begin{corollary}[Consistency~\cite{andersen1982cox}] If $\LL(\w,\f)$ attains unique maximizer in $\W$ then $\widehat \w \overset{p}{\to} \w^*$. 
% % With compact parameter space, continuity of the objective function, uniform convergence, and unique maxima, the MLL estimator is consistent.
% \end{corollary}

% \todoy[inline]{make this example better fit into the context}
 
Having provided sufficient conditions,  
we consider a binary classification example
to provide intuition for why we need calibration for consistency.
In this example, we relate the estimation error to the miscalibration error,
showing that calibration is not only sufficient but also necessary
to achieve zero estimation error for a certain class of predictors. 
% 
% 
% with a simple Gaussian mixture model. 
% 
% 
% \begin{restatable}[]{reex}{necessary}
% \label{ex:necessary}
% Consider a mixture of two Gaussians with 
% \allowdisplaybreaks{$\ps(x|y=0) \defeq \N(\mu, 1)$ 
% and $\ps(x|y=1) \defeq \N(-\mu, 1)$}. 
% Assume that source mixing coefficients are both $\frac{1}{2}$
% and that target mixing coefficients are $\alpha (\ne \frac{1}{2}), 1-\alpha $. 
% Assume a class of probabilistic threshold classifiers:
% $f(x) = [1-c, c]$ for $x\ge 0$, otherwise $f(x) = [c, 1-c]$ with $c \in [0,1]$.
% % $f(x) = [ \frac{1+(2c-1)\sign(x)}{2}, \frac{1-(2c-1)\sign(x)}{2}]$ with $c \in [0,1]$.  
% The population error of MLLS is given by 
% $
% %4\abs{\frac{\pt(x\le0) - c}{1-2c} - \alpha} =
% 4\abs{\frac{(1-2\alpha)(\ps(x\ge0|y=0) - c)}{1-2c}}$ 
% which is zero only if $c = \ps(x\ge0|y=0)$ for a non-degenerate classifier. 
% \end{restatable}


\textbf{Example 1.} Consider a mixture of two Gaussians with 
\allowdisplaybreaks{$\ps(x|y=0) \defeq \N(\mu, 1)$ 
and $\ps(x|y=1) \defeq \N(-\mu, 1)$}. 
We suppose that the source mixing coefficients are both $\frac{1}{2}$, while
the target mixing coefficients are $\alpha (\ne \frac{1}{2}), 1-\alpha $. 
Assume a class of probabilistic threshold classifiers:
$f(x) = [1-c, c]$ for $x\ge 0$, otherwise $f(x) = [c, 1-c]$ with $c \in [0,1]$.
% 
% $f(x) = [ \frac{1+(2c-1)\sign(x)}{2}, \frac{1-(2c-1)\sign(x)}{2}]$ with $c \in [0,1]$.  
Then the population error of MLLS is given by 
%4\abs{\frac{\pt(x\le0) - c}{1-2c} - \alpha} =
\begin{align*}
4\abs{\frac{(1-2\alpha)(\ps(x\ge0|y=0) - c)}{1-2c}},
\end{align*}
which is zero only if $c = \ps(x\ge0|y=0)$ for a non-degenerate classifier.

% We extend the construction to probabilistic thresholded classifier in Appendix-\ref{sec:AppendixA}.   

% Why such construction: 
%The intuition behind the construction is, for such problems, we can get a closed form expression for the population MLLS estimator and hence analyse the error theoretically. 
The expression for estimation error arising from our example yields two key insights:
% The main take away from this example is 
(i) an uncalibrated thresholded classifier has an estimation error 
proportional to the true shift in label distribution  i.e. $1-2\alpha$;
(ii) the error is also proportional to the 
canonical calibration error which is $\ps(x\ge0|y=0) - c$. 
% We formally derive the expression for 
% estimation error in Appendix~\ref{sec:AppendixA}. 
% 
While earlier in this section, we concluded 
that canonical calibration is sufficient for consistency,
the above example provides some intuition 
for why it might also be necessary. 
In Appendix~\ref{ref:marg_calib}, we show that marginal calibration~\citep{kumar2019verified,guo2017calibration,vaicenavicius2019evaluating}, a less restricted definition is insufficient to achieve consistency. % OK
% but we leave a formal characterisation of necessary conditions for future work.
% \todos{Here we can include the proof for necessity?}

\vspace{-5pt}
\subsection{MLLS with Confusion Matrix} \label{subsec:MLLS_CM}
\vspace{-3pt}

So far, we have shown that MLLS with any calibrated predictor 
can be viewed as distribution matching in a latent space. 
Now we discuss a method to construct a predictor $\f$ 
to perform MLLS given any $p(\z|\x)$, e.g.,
those induced by confusion matrix approaches. 
Recall, we already have the maximum log-likelihood objective.
% given any $p(\z|\x)$ in \eqref{eq:mlls-z}, 
It just remains to construct a calibrated predictor $\f$ from the confusion matrix. 
% such that 
% one can rewrite  as \eqref{eq:mlls-main}. 


This is straightforward when $p(\z|\x)$ is deterministic, i.e.,
$p(\z|\x) = \delta_{g(\x)}$ for some function $g$: 
setting $\f(\x) = p_s(y|g(\x))$ makes the objectives \eqref{eq:mlls-z} and \eqref{eq:mlls-main} to be the same. 
% 
Recall that for the hard confusion matrix,
the induced latent space is 
$p(\z|\x) = \delta_{\argmax \widehat{\f}(\x)}$.
So the corresponding predictor in MLLS is $\smash{\f(\x) = p_s(y|\widehat{y}_{\x})}$,
where $\smash{\widehat{y}_{\x} = \argmax \widehat{\f}(\x)}$.
Then we obtain the MLLS objective for the hard confusion matrix:
\vspace{-5pt}
\begin{align*}
\max_{w \in \W} \EE{t}{ \log \sum\nolimits_{y=1}^k p_s(y|\widehat{y}_{\x})  \w_y} \,.
\addeq\label{eq:cm-log} 
\end{align*}
The confusion matrix $\smash{\C_{\widehat{\f}}}$ and predictor $\smash{\widehat{\f}}$
directly give us $\smash{p_s(y|\widehat{y}_{\x})}$. Given an input $\x$, one can first get $\widehat{y}_{\x}$ from $\widehat{\f}$, 
then normalize the $\widehat{y}_{\x}$-th row of $\C_{\widehat{\f}}$ as $p_s(y|\widehat{y}_{\x})$.  We denote MLLS with hard confusion matrix calibration \eqref{eq:cm-log} by MLLS-CM. %is directly accessible from the confusion matrix 
% $\C_{\widehat{\f}}$ 
% along with the black box predictor $\widehat{\f}$: 

When $p_s(\z|\x)$ is stochastic, we need to extend \eqref{eq:mlls-main} to allow $\f$ to be a random predictor: 
$\f(\x)=p_s(y|\z)$ for $\z\sim p(\z|\x)$\footnote{Here, by a random predictor we mean that the predictor outputs a random vector from $\Delta^{k-1}$, not $\out$.}.
To incorporate the randomness of $\f$,
one only needs to change the expectation in \eqref{eq:mlls-main} to be over both $\x$ and $\f(\x)$,
then \eqref{eq:mlls-main} becomes a rewrite of \eqref{eq:mlls-z}. 
% 
% Again, the random predictor is calibrated 
% and we can have an MLLS objective 
% for the soft confusion matrix approach.
% 

Proposition~\ref{prop:ltt-calib} indicates that constructing 
the confusion matrix is a calibration procedure.
% for any black box predictor $\smash{\widehat{\f}}$, 
% one can obtain a calibrated predictor $\f$ from its confusion matrix $\smash{\C_{\widehat{\f}}}$. 
% \todos{I have done some heavy cutting here, please give it a read aand see if this makes sense.}
Thus, the predictor constructed with constructed using confusion matrix is calibrated
and suitable for application with MLLS.
% See Appendix~\ref{subsec:MLLS_soft} for more details.
% 
% on the construction procedure with soft confusion matrix. 
% 
% For MLLS objective constructed in this way, 
% the predictor is also calibrated:
% Using this predictor, MLLS is consistent. 
\begin{restatable}[\citet{vaicenavicius2019evaluating}]{reprop}{recalib}\label{prop:ltt-calib}
For any function $g$, $\f(\x) = p_s(y|g(\x))$ is a calibrated predictor.
% \vspace{-5pt}
\end{restatable}

%\footnote{See Appendix for details.} 

We can now summarize the relationship between BBSE and MLLS:
A label shift estimator involves two design choices: 
(i) designing the latent space $p(\z|\x)$ 
(which is equivalent to designing a calibrated predictor); 
and (ii) performing distribution matching
in the new space $\ltt$. 
In BBSE, we design a calibrated predictor 
via the confusion matrix
and then perform distribution matching 
by directly solving linear equations. 
In general, MLLS does not specify 
how to obtain a calibrated predictor, 
but specifies KL minimization as 
the distribution matching procedure.
One can apply the confusion matrix approach 
to obtain a calibrated predictor 
and then plug it into MLLS, 
which is the BBSE analog under MLLS, 
and is a special case of MLLS.

==> sections/finite.tex <==
 \label{sec:finite}
 
We now analyze the MLLS estimators' convergence rates. For detailed proof from this section, we refer reader to Appendix \ref{sec:AppendixB}. 
Recall ${\widehat \w}$ denotes MLLS estimate~\eqref{eq:mlls-sample}. 
Let ${\w}^*$ denote the true shift. With consistency condition from section~\ref{subsec:MLLS}, we assume that $\w^*$ is the population minimizer with the calibrated predictor $\fc =  \ProbS({ y= . | \widehat \f(\x) })$ .i.e. 
\begin{align}
\w^* = &\argmax_{w \in \W} \E{\LL(\w; \fc )} \label{eq:MLLS_fc}
% &\quad \text{s.t.} \quad \sum_{y=1}^{k} w(y)\ps(y) = 1 \numberthis 
% &\quad \qquad \forall y \in \out \quad w(y) \ge 0 
\end{align}
 Our goal is to bound the finite sample error:  
\begin{equation}\label{eq:err}
    \Delta_n = ||\widehat \w - \w^*||_2 \le  \underbrace{||\widehat \w - \wc||_2}_{\RN{1}} +  \underbrace{||\wc - \w^*||_2}_{\RN{2}}  
\end{equation} 
where $ \wc$ is the finite sample estimation with the perfectly calibrated predictor $\fc$. We bound each error term on the RHS individually. Term-$\RN{1}$ denotes the estimation error due to finite sample re-calibration or inherent model misscalibration and term-$\RN{2}$ is the finite sample error with a perfectly calibrated model. 

% We use the following lemma
% % ~\ref{lemma:err_1} 
% to bound the error term-$\RN{2}$:  

\begin{lemma}[Error bound on term-$\RN{2}$]\label{lemma:err_1}
Assume the identifiability condition of lemma~\ref{lemma:identi-1} hold true and the predictor function  $\fc$ is bounded below at the non zero entries of $\w^*$ i.e. for all $\x$ such that $\pt(\x)>0$, we have $\sum_{y=1}^k \fc_y(\x) \w^*_y \ge \tau$ for some universal constant $\tau$. Let $\smin^{\fc}$ be the minimum eigenvalue of the Fisher information.  With probability at least $1-\delta$ we have,  
$$||\wc - \w^*||_2 \defeq \comp \left(\frac{1}{\smin^{\fc}}\sqrt{\frac{\log(\frac{4}{\delta})}{m}}\right)$$
\end{lemma}

\begin{proofsketch}

\end{proofsketch}


\begin{lemma}[Error bound on term-$\RN{1}$] \label{lemma:err_2}
Assume conditions from lemma \ref{lemma:err_1} hold true. Additionally assume the learnt predictor $\fh$ is also bounded below at the non zero entries of $\w^*$ i.e. for all $\x$ such that $\pt(\x)>0$, we have $\sum_{y=1}^k \fh_y(\x) \w^*_y \ge \tau$ for some universal constant $\tau$. Let $\smin^{\fh}$ be the minimum eigenvalue of the Fisher information with predictor $\fh$. With probability at least $1-\delta$ we have, 
\[
 || \wc - \widehat \w ||_2 \defeq \comp \left( \frac{1}{\sigma_{\min}^{\fh}}\Big(\sqrt{\frac{\log(\frac{4}{\delta})}{m}} +  \CE{\fh}||\w^*||_2 \Big) \right)
\]
\end{lemma}
\begin{proofsketch}

\end{proofsketch}

Depending on the degree of the miscalibration and method involved to calibrate $\fh$ we can bound the $\CE{\widehat \f}$. For example, if using vector scaling on a held out validation data from source for calibration, we can use lemma-\ref{lemma:platt} from Appendix \ref{sec:AppendixB} to bound the calibration error $\CE{\widehat \f}$ i.e. with standard regularity assumptions on model class $\G$ used for calibration we have with probability at least $1-\delta$,  
\begin{equation} \label{eq:platt}
  \CE{\fh} \le  \min_{\g \in \G} \CE{\g \circ \fh } + \sqrt{c\frac{\log(\frac{2}{\delta})}{n}}  
\end{equation}
  
\begin{theorem}[Error bounds] \label{thm:err}
Assume identifiability conditions of lemma \ref{lemma:identi-1} and assumption A.1 hold true. With probability at least $1-\delta$ we have, 
\begin{equation*}
\begin{split}
||\widehat \w - \w^*||_2  \defeq \comp \Bigg(\frac{1}{\smin^{\fc}}\sqrt{\frac{\log(\frac{4}{\delta})}{m}}  &+ \frac{1}{\sigma_{\min}^{\fh}}\Big(\sqrt{\frac{\log(\frac{4}{\delta})}{m}} \\ &+ \CE{\fh}||\w^*||_2 \Big) \Bigg)
\end{split}
\end{equation*}

\end{theorem}
The proof follows simply by combining above lemma's bounding the error terms $\RN{1}$ and $\RN{2}$ in \eqref{eq:err}. 

\todos[inline]{Remarks and takeaways from the above lemmas and theorem.}

\todos[inline]{Re-define the assumption from lemmas and justify that.}
To derive the finite sample bounds in lemma \ref{lemma:err_1} and \ref{lemma:err_2}, we make the following assumption: 

(A.1) \quad  


\textbf{Justification.} 
 
 
\todos[inline]{Explain what happens on the boundary} 

We begin this section by showing strong convexity of the log-likelihood. We need this condition for all our finite sample error analysis.

\begin{prop} \label{prop:strongconcave}
With the identifiability of the log-likelihood, the optimization problem~\eqref{eq:mlls-sample} is strongly convex.  
\end{prop}

The proof argument is detailed in Appendix-\ref{sec:AppendixB} the identifiability assumption. 


% \subsection{Generalization results} 
\todos{Majorly these will be from kamyar's paper which can be included for completeness.}


==> sections/theory.tex <==
This section discusses our theoretical results -- 
% (i) we analyze the properties of the likelihood function, 
(i) necessary and sufficient conditions for consistency of MLLS, and (ii) finite sample error bounds for MLLS.  


The log-likelihood of observing \allowdisplaybreaks{$ \x_1, \x_2, \ldots, \x_m \stackrel{iid}{\sim} \pt(x)$} under the true model is given by 
%\todos[inline]{We can possibly shift this to appendix.}
\begin{align*}
\LL_m(\w, \f^*) &= \sum_{i=1}^m \log \pt(\x_i)\\
&\stackrel{i}{=} \sum_{i=1}^m \log \sum_{y\in\out} \pt(\x_i|y)\pt(y)   \\
&\stackrel{ii}{=} \sum_{i=1}^m \log \sum_{y\in\out} \ps(\x_i|y)\pt(y) \\
&= \sum_{i=1}^m \log \sum_{y\in\out} \ps(y|\x_i)\frac{\pt(y)}{\ps(y)} + \sum_{i=1}^m \log p_s(\x_i)
\end{align*}

where $(i)$ follows with Bayes theorem and $(ii)$ follows due to the label shift assumption. From now on, we ignore the term $\sum_{i=1}^m \log p_s(\x_i)$ as it is independent of the underlying parameters. 
We refer population log-likelihood as $\LL(\w, \f) = \E{\log\inner{\f(\x)}{\w} }$ and define the empirical log-likelihood as \allowdisplaybreaks{$\LL_m(\w; \widehat \f) =  \sum_{i=1}^m \log \sum_{y\in\out} \widehat \ps(y|\x_i)w(y) = \sum_{i=1}^m \log \inner{\widehat \f(\x_i)}{\w} $} which uses the predictor function $\widehat \f$ instead of the true marginal distribution.

We estimate the weights $\w$  i.e. the shift in the label distribution by maximizing the empirical log-likelihood (or minimizing the negative log-likelihood) 
\begin{align*}
\widehat \w = &\argmin_w - \LL_m(\w; \widehat \f ) \\ 
&\quad \text{s.t.} \quad ~\sum_{y=1}^{k} w(y)\ps(y) = 1 \numberthis \label{optprob}\\ 
&\quad \qquad \forall y \in \out \quad w(y) \ge 0 
\end{align*}

The above optimization problem is convex in nature as shown below. 
Under the assumption of non-zero support of source labels i.e. for all $y \in \out$ $\ps(y) = c > 0$ , the likelihood objective is also bounded above by $-\log(c)$. 
% In Appendix~\ref{sec:AppendixB}, we also show that the optimization problem is also self concordant (Proposition~\ref{prop:sc}). 
\begin{prop} The optimization problem defined in \eqref{optprob} is convex in nature.
\end{prop}
The proof argument follows simply. The objective function is negative log, a convex combination of a linear function in parameters. The minimization is over a convex region i.e. a simplex of dimensions $k-1$, and hence the overall optimization problem is convex.   

\textbf{Methods to maximise the likelihood.}
The optimization problem defined in \eqref{optprob} doesn't  
% Want to connvey unsurety 
seem to have a closed form solution but due to convexity and upper boundedness, we can use iterative procedures to find the MLLS estimate. In particular, we employ Expectation Maximisation (EM)~\cite{saerens2002adjusting} and mirror descent~\cite{beck2003mirror} on the likelihood function and observe same estimates empirically at the convergence of the iterates.    


% \todos{Ask if we should include formulation of EM and mirror descent. If needed I can add those.}

\subsection{Consistency of the estimate}\label{subsec:consistency}
In this subsection we formalize conditions on the predictor function $\widehat \f$ under which the optimization objective~\eqref{optprob} is identifiable, and the corresponding MLLS estimate is consistent.  

% \textbf{Motivating Scenario.}
% We begin with an example of binary classification problem on a mixture of two Gaussians where we show that calibration is necessary to achieve zero estimation error. To motivate the need for calibration we relate estimation error with the miscalibration error.  
% % with a simple Gaussian mixture model. 


% \begin{example} \label{ex:necessary}
% Consider a mixture of two Gaussians with \allowdisplaybreaks{$\ps(x|y=0) \defeq \N(\mu, 1)$ and $\ps(x|y=1) \defeq \N(-\mu, 1)$}. Assume source mixing coefficients be $\frac{1}{2}$ each and target mixing coefficients be $\alpha (\ne \frac{1}{2}), 1-\alpha $. Assume a class of probabilistic classifiers with threshold at $x=0$ that can be represented as $f(x) = [ \frac{1+(2c-1)\sign(x)}{2}, \frac{1-(2c-1)\sign(x)}{2}]$ with $c \in [0,1]$.  For such classifiers, the estimation error of population MLLS is given by $4\abs{\frac{\pt(x\le0) - c}{1-2c} - \alpha} = 4\abs{\frac{(1-2\alpha)(\ps(x\ge0|y=0) - c)}{1-2c}}$ which is zero for only if $c = \ps(x\ge0|y=0)$ for a non-degenerate classifier. 
% \end{example}

% % We extend the construction to probabilistic thresholded classifier in Appendix-\ref{sec:AppendixA}.   

% % Why such construction: 
% The intuition behind the construction is, for such problems, we can get a closed form expression for the population MLLS estimator and hence analyse the error theoretically. The expression for estimation error in the example gives two key insights; 
% % The main take away from this example is 
% One, uncalibrated thresholded classifier has an estimation error proportional to the true shift in label distribution  i.e. $1-2\alpha$.
% and two, the error is also proportional to degree of miscalibration which is $\ps(x\ge0|y=0) - c$. We formally derive the expression for estimation error in Appendix-\ref{sec:AppendixA}. 

% In the example below, we show that for any shift in the label distribution estimation error of the population MLLS estimator is directly propotional to the miscalibration error of the predictor function. 
% This gives some intuition on why calibration might be necessary but we leave a formal proof for this argument as future work.  

We now turn our discussion to
sufficient 
conditions for consistency.
\todos[inline]{I am not editing remaining of the subsection right now. We can discuss and decide what I should edit in this subsection.}

% \begin{prop}\label{prop:ident}
% (Identifiability condition.) Log-likelihood \allowdisplaybreaks{$\LL_m(\w; \widehat \f )$} is identifiable iff the matrix \allowdisplaybreaks{$\mathrm{\widehat P} = [\widehat \f(\x_1) \ldots \widehat \f(\x_n)]_{(k\times n)}$} formed by considering $\widehat \f(\x_i|y)$ for all $i\in \{1,\ldots,n\}$ and $y \in \out$ in the training data is full row-rank\footnote{Be default we assume we observe samples n greater than number of classes $\abs{\out}$}.
% \end{prop}
% % \todos[inline]{Ask how to handle continuos cases. }
% \begin{proof}
% Let's assume $\bm{q_1}, \bm{q_2}$ be vectors lying in $k-1$ dimentional simplex. With identifiability condition, if \allowdisplaybreaks{$ \bm{q_1} \ne \bm{q_2}$} then it must be the case that $\widehat \LL (\w_1; \x) \ne \widehat \LL_m(\w_2; \x)$. 

% Consider any arbitrary set $\x_1, \ldots, \x_n$ in the training data, log-likelihoods can only match when \allowdisplaybreaks{$[\widehat \f(\x_1) \ldots \widehat \f(\x_n)]^T \bm{q_1} = [\widehat \f(\x_1) \ldots \widehat \f(\x_n)]^T  \bm{q_2}$}. 
% Hence by rank-nullity theorem, full row-rank $\mathrm{\widehat P}$ implies identifiability.  
% \end{proof}
% \todos[inline]{I can add a detailed proof if it is required. We just need to add justification for what will happen if $\pt(x)$ is zero for some x. }

As the parameter $\w$ is restricted to a compact set, proposition
% -\ref{prop:ident} 
also implies strong identifiability.
% ~\cite{lecturenotes}. 
Full rank of $\mathrm{\widehat P}$ is also implied by full rank of the confusion matrix considered in \cite{lipton2018detecting}, but identifiability requires a weaker condition. 
Similar to proposition
% -\ref{prop:ident}
, we also need identifiability on the true log-likelihood which requires the true predictor function $\ps(y|\x)$ to be full rank on the source data. 


For consistency, we also need uniform law of large numbers condition on the log-likelihood which boils down to showing decaying Rademacher complexity on the approximate log-likelihood function class
% ~\cite{lecturenotes}
. We detail this argument in the appendix \ref{sec:AppendixA}.  

% \begin{lemma}\label{lemma:RC} (Rademacher complexity) Under certain assumptions viz.  boundedness etc. on the predictor function $\widehat \f$, the Rademacher complexity is 
% \begin{align*}
%  \R(\LL_m(\widehat \f )) = \mathbb{E}_{\x,\epsilon} &\Big[ \sup_{\w} \frac{1}{n} \sum_{i=1}^n \epsilon_i \log \inner{\widehat \f(\x_i)}{\w}  \Big] \\
%  &\defeq \comp(\frac{1}{\sqrt{m}})
% \end{align*}
% \end{lemma}

% \begin{lemma} [\cite{lecturenotes} Uniform LLN] As the log-likelihood function is continuous over the closed and bounded space of weight parameters and $\E{\sup_{\w} |\L_1(\x, \w ,\f)|}$ exists\footnote{This is finite for all $\w$'s that have a support for all non-zero $\w^*$'s}, we have uniform convergence on the empirical log-likelihood. 

% \end{lemma}



\begin{lemma}[Uniform Convergence~\cite{andersen1982cox}] \label{lemma:uc}
Suppose a sequence of convex function $\LL_m(\w, \f)$ converges in probability to $\LL(\w, \f)$ for $w$ in an open set $\mathcal{W}$, then $\sup_{\mathcal{W}^\prime} \abs{\LL_m(\w, \f) - \LL(\w, \f)}$ goes to zero in probability on every compact subset $\mathcal{W}^\prime$ of $\mathcal{W}$.     
\end{lemma}


\begin{lemma} [Consistency] With compact parameter space, continuity of the objective function, uniform convergence, and unique maxima, the MLL estimator is consistent.
\end{lemma}
\todos{For unique maxima we need identiability on the source data i.e. the predictor matrix being invertible. }


% Refer to Appendix~\ref{sec:AppendixA} for proof details. The argument uses Lipschitzness property and composition of Rademacher complexity. 

In any practical setting, with finite amount of data we can never estimate the true predictor $\ps(y|x)$ which leads to misspecified likelihood model. Thus, at the population level the MLE estimate would be the KL projection of true data generating distribution on our model.
% ~\cite{lecturenotes}. 
With per label calibration of the predictor function on the source data, we show that such model mis-specification is harmless. 
% First we give the definition of the \textit{per-label calibration} and then show the consistency of the MLE estimate.  


\begin{lemma} \label{lemma:consistency}
Suppose a predictor $\f$ is per-label calibrated and some identifiability condition, then true model $\LL (\w^*, \f^*)$ lies in the model class $\LL (\w, \f) $.
\end{lemma}
\begin{proof}
\todos[inline]{Add proof for the binary case}

\todos[inline]{Add the full-rank assumption of $\ps(\f(\x)|y)$ for identifiability.}
\end{proof}

In  Appendix \ref{sec:AppendixA}, we extend the proof to multiclass classification with continuos probabilities. \todos{Discuss with Yifan and add. }  

\begin{theorem}\label{theorem:con}
Assume per-label calibration and likelihood identifiability conditions hold, then the MLE is consistent. 
\end{theorem}  

% The proof follows by combining proposition~\ref{prop:ident}, lemma~\ref{lemma:RC}, and lemma~\ref{lemma:consistency}. The proof is formally compiled in Appendix \ref{sec:AppendixA}. 

We conclude that calibration is sufficient for consistency. Example-\ref{ex:necessary} gives intuition on why calibration might also be necessary but we leave a formal proof for this argument as future work.  
% \begin{example}\la
% Consider a mixture of Gaussian with \allowdisplaybreaks{$\ps(x|y=1) \defeq \N(1, 1)$ and $\ps(x|y=-1) \defeq \N(-1, 1)$}. Let source mixing coefficients be $\frac{1}{2}$ each and $\alpha, 1-\alpha$ be the target mixing coefficients. With any thresholded classifier of the form $f(x) = [ \frac{1+\sign(x)}{2}, \frac{1-\sign(x)}{2}]$, the estimation error is $4\abs{\pt(x\ge0) - \alpha} = 4\times 0.1587\abs{1 - 2\alpha}$ which is non-zero for all $\alpha \ne \frac{1}{2}$
% \end{example}


\subsection{Unified View}\label{subsec:unified}

Rather, one could also incorporate the predictor generated using the confusion matrix which in principle is calibrated (Proposition~\ref{prop:calib}). In section ~\ref{sec:exp}, we contrast this predictor with the one obtained with vector scaling and evaluate the loss information caused to due aggregation of predictions in terms of the Fisher information of our log-likelihood.
\todos{Ask how to pitch this? In general how to present this section?}

\begin{prop}\label{prop:calib}
Confusion matrix using a predictor $f$ in principle gives a per-label calibrated classifier on the source data. 
\end{prop}
The proof is in Appendix~\ref{sec:Appendixbgr}, which follows from the construction of confusion matrix and Definition~\ref{def:calib}.

\subsection{Finite sample error analysis} \label{subsec:finite}
% \todos[inline]{OK, so, all proofs go through for the positive support of $w^*$ and we can extrapolate for zero support with lemma-\ref{lemma:support}.}
 
We now analyze the MLLS estimators' convergence rates. For detailed proof from this section, we refer reader to Appendix \ref{sec:AppendixB}. 
Recall ${\widehat \w}$ denotes MLLS estimate~\eqref{optprob}. 
Let ${\w}^*$ denote the true shift. With consistency condition from section~\ref{subsec:consistency}, we assume that $\w^*$ is the population minimizer with the calibrated predictor $\fc =  \ProbS({ y= . | \widehat \f(\x) })$ .i.e. 
\begin{align}
\w^* = &\argmin_{w \in \W} - \E{\LL(\w; \fc )} \label{eq:MLLS_fc}
% &\quad \text{s.t.} \quad \sum_{y=1}^{k} w(y)\ps(y) = 1 \numberthis 
% &\quad \qquad \forall y \in \out \quad w(y) \ge 0 
\end{align}
 Our goal is to bound the finite sample error:  
\begin{equation}\label{eq:err}
    \Delta_n = ||\widehat \w - \w^*||_2 \le  \underbrace{||\widehat \w - \wc||_2}_{\RN{1}} +  \underbrace{||\wc - \w^*||_2}_{\RN{2}}  
\end{equation} 
where $ \wc$ is the finite sample estimation with the perfectly calibrated predictor $\fc$. We bound each error term on the RHS individually. Term-$\RN{1}$ denotes the estimation error due to finite sample re-calibration or inherent model misscalibration and term-$\RN{2}$ is the finite sample error with a perfectly calibrated model. 

% We use the following lemma
% % ~\ref{lemma:err_1} 
% to bound the error term-$\RN{2}$:  

\begin{lemma}[Error bound on term-$\RN{2}$]\label{lemma:err_1}
Assume the identifiability condition of lemma~\ref{lemma:identi-1} hold true and the predictor function  $\fc$ is bounded below at the non zero entries of $\w^*$ i.e. for all $\x$ such that $\pt(\x)>0$, we have $\sum_{y=1}^k \fc_y(\x) \w^*_y \ge \tau$ for some universal constant $\tau$. Let $\smin^{\fc}$ be the minimum eigenvalue of the Fisher information.  With probability at least $1-\delta$ we have,  
$$||\wc - \w^*||_2 \defeq \comp \left(\frac{1}{\smin^{\fc}}\sqrt{\frac{\log(\frac{4}{\delta})}{m}}\right)$$
\end{lemma}

\begin{proofsketch}

\end{proofsketch}


\begin{lemma}[Error bound on term-$\RN{1}$] \label{lemma:err_2}
Assume conditions from lemma \ref{lemma:err_1} hold true. Additionally assume the learnt predictor $\fh$ is also bounded below at the non zero entries of $\w^*$ i.e. for all $\x$ such that $\pt(\x)>0$, we have $\sum_{y=1}^k \fh_y(\x) \w^*_y \ge \tau$ for some universal constant $\tau$. Let $\smin^{\fh}$ be the minimum eigenvalue of the Fisher information with predictor $\fh$. With probability at least $1-\delta$ we have, 
\[
 || \wc - \widehat \w ||_2 \defeq \comp \left( \frac{1}{\sigma_{\min}^{\fh}}\Big(\sqrt{\frac{\log(\frac{4}{\delta})}{m}} +  \CE{\fh}||\w^*||_2 \Big) \right)
\]
\end{lemma}
\begin{proofsketch}

\end{proofsketch}

Depending on the degree of the miscalibration and method involved to calibrate $\fh$ we can bound the $\CE{\widehat \f}$. For example, if using vector scaling on a held out validation data from source for calibration, we can use lemma-\ref{lemma:platt} from Appendix \ref{sec:AppendixB} to bound the calibration error $\CE{\widehat \f}$ i.e. with standard regularity assumptions on model class $\G$ used for calibration we have with probability at least $1-\delta$,  
\begin{equation} \label{eq:platt}
  \CE{\fh} \le  \min_{\g \in \G} \CE{\g \circ \fh } + \sqrt{c\frac{\log(\frac{2}{\delta})}{n}}  
\end{equation}
  
\begin{theorem}[Error bounds] \label{thm:err}
Assume identifiability conditions of lemma \ref{lemma:identi-1} and assumption A.1 hold true. With probability at least $1-\delta$ we have, 
\begin{equation*}
\begin{split}
||\widehat \w - \w^*||_2  \defeq \comp \Bigg(\frac{1}{\smin^{\fc}}\sqrt{\frac{\log(\frac{4}{\delta})}{m}}  &+ \frac{1}{\sigma_{\min}^{\fh}}\Big(\sqrt{\frac{\log(\frac{4}{\delta})}{m}} \\ &+ \CE{\fh}||\w^*||_2 \Big) \Bigg)
\end{split}
\end{equation*}

\end{theorem}
The proof follows simply by combining above lemma's bounding the error terms $\RN{1}$ and $\RN{2}$ in \eqref{eq:err}. 

\todos[inline]{Remarks and takeaways from the above lemmas and theorem.}

\todos[inline]{Re-define the assumption from lemmas and justify that.}
To derive the finite sample bounds in lemma \ref{lemma:err_1} and \ref{lemma:err_2}, we make the following assumption: 

(A.1) \quad  


\textbf{Justification.} 
 
 
\todos[inline]{Explain what happens on the boundary} 

We begin this section by showing strong convexity of the log-likelihood. We need this condition for all our finite sample error analysis.

\begin{prop} \label{prop:strongconcave}
With the identifiability of the log-likelihood, the optimization problem~\eqref{optprob} is strongly convex.  
\end{prop}

The proof argument is detailed in Appendix-\ref{sec:AppendixB} the identifiability assumption. 


% \subsection{Generalization results} 
\todos{Majorly these will be from kamyar's paper which can be included for completeness.}

